Fearless Asynchronous Communications with Timed Multiparty Session Protocols

Session types using affinity and exception handling mechanisms have been developed to ensure the communication safety of protocols implemented in concurrent and distributed programming languages. Nevertheless, current affine session types are inadequate for specifying real-world asynchronous protocols, as they are usually imposed by time constraints which enable timeout exceptions to prevent indefinite blocking while awaiting valid messages. This paper proposes the first formal integration of affinity, time constraints, timeouts, and time-failure handling based on multiparty session types for supporting reliability in asynchronous distributed systems. With this theory, we statically guarantee that asynchronous timed communication is deadlock-free, communication safe, while being fearless -- never hindered by timeout errors or abrupt terminations. To implement our theory, we introduce a Rust toolchain designed to facilitate the implementation of safe affine timed protocols. Our toolchain leverages generic types and the time library to handle timed communications, integrated with optional types for affinity. We evaluate our approach by extending diverse examples from the literature to incorporate time and timeouts, demonstrating that our solution incurs negligible overhead compared with an untimed implementation. We also showcase the correctness by construction of our approach by implementing various real-world use cases, including a remote data protocol from the Internet of Remote Things domain, as well as protocols from real-time systems like Android motion sensors and smartwatches.

==> conclusion.tex <==
\subsection{Conclusion and future work}
\label{sec:conclusion}









As future work,
we can extend~\timedmulticrusty
to extract the graphs from
the local endpoints to
check the~\emph{Multiparty-compatiblity},
guided by~\citet{lange2019Verifying}
and their tool~\kmc.
In line with this approach,
usually called~\emph{bottom-up},
it could be interesting to
extend~\timedmulticrusty to
handle asynchronous communications
with buffers:
messages may be sent or received out
of order,
and~\timedmulticrusty
should be able to check
such protocols.
We could also propose
a way to recover from errors
instead of simply kill
the processes,
as proposed by~\citet{neykova2017timed}.

==> evaluations_short.tex <==
\section{Evaluations: benchmarks, expressiveness and case studies}
\label{sec:evaluation}
We evaluate our toolchain from two perspectives: \emph{expressivity} and \emph{feasibility}.
For expressiveness,
we implement protocols provided in the session type literature~\cite{hu2016Hybrid,neykova2013Spy,fielding2014Hypertext,jia2016Monitors,huSessionBased2008}, as well as protocols from real-time systems~\cite{androidMotionSensors,Pine64,propositions2012Wadler},
inspired by~\cite{DBLP:journals/pacmpl/IraciandCHZ2023}.
For feasibility, comparing to~\multicrusty, which is an untimed implementation
of affine synchronous \MPST,
we show that our system
exhibits minimal compile-time overhead in all cases,
and minimal runtime overhead except for three cases due the huge number of time constraints.












\emph{Setup.}
To perform the benchmarking,
we configure \criterionRust \cite{web:rust:criterion}
to use bootstrap sampling
\cite{dixon2006bootstrap,efron1992bootstrap}
on each protocol,
with samples of size 100,000,
then report the average execution time
with a confidence interval of 95\%.
Additionally,
we benchmark the compilation time by compiling
each protocol 100 times and reporting the mean.
To compile,
we use the commands \CODE{cargo clean} and \CODE{cargo build [name of the file]}.
The \CODE{cargo clean} command removes all compiled files,
including compiled dependencies,
while the second command,
without any additional parameters,
compiles the given file and its dependencies
without optimising the resulting files.
The machine configuration we use is a workstation with an
Intel\textregistered~
Core\texttrademark~
i7-7700K CPU @ 4.20 GHz
with 8 threads and 32 GB of RAM,
Manjaro Linux 23.0.2,
Linux kernel 6.1.53-1,
along with the latest versions of
\rustup (1.26.0) and the \Rust cargo compiler (1.73.0).





\subsection{Performance Comparison Between~\timedmulticrusty and~\multicrusty}
\label{subsec:evaluation:benchmarks}




















Comparing \timedmulticrusty and \multicrusty,
we assessed their performance on two protocols:
the \emph{ring} and \emph{mesh} protocols.
The ring protocol involves passing a message sequentially through roles,
while the mesh protocol requires each participant to send a message to every other.
Both protocols underwent 100 iterations within a $0$ and $10$-second time window.
Benchmark results,
ranging from 2 to 8 roles,
are presented in \Cref{fig:benchmark_results_examples} (top),
with \multicrusty denoted as \AMPST and \timedmulticrusty as \ATMP.



In the \emph{ring} protocol (\Cref{appendix:subfig:ring_protocol}),
compile-time benchmarks (\Cref{fig:benchmark_results:compile:ring})
show \timedmulticrusty marginally slower at 2 roles (less than 2\%)
and around 5\% faster at 8 roles.
The runtime benchmarks (\Cref{fig:benchmark_results:running:ring})
exhibit a 15\% speed advantage for \multicrusty at 2 roles,
diminishing to 5\% at 8 roles.
The overhead remains consistent,
with less than 0.5 ms difference at 6,
7,
and 8 roles.



The \emph{mesh} protocol (\Cref{appendix:subfig:mesh_protocol})
involves all roles sending and receiving messages
(\Cref{fig:benchmark_results:compile:mesh} for compile-time,
\Cref{fig:benchmark_results:running:mesh} for runtime).
Similar to the ring protocol,
\timedmulticrusty compiles slightly slower (less than 1\% at 2 roles,
4\% at 8 roles) and runs slower (less than 1\% at 2 roles,
15\% at 8 roles).
\timedmulticrusty's compile times range from 18.9 s to 26 s,
with running times between 0.9 ms and 11.9 ms.
The gap widens exponentially due to the increasing number of enforced time constraints.



In summary,
\timedmulticrusty exhibits overhead compared to \multicrusty,
increasing with the number of roles.
This can be attributed to additional features in \timedmulticrusty,
such as eight parameters for time constraints,
compared to \multicrusty's two.
Despite this,
\timedmulticrusty's enhanced capabilities for asynchronous
and timed communications result in overall manageable overheads.



















\subsection{Case Studies}
\label{subsec:evaluation:examples}





\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.026\textwidth}
        \includegraphics[width=\textwidth, height=7em]{pdf/time_seconds.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth, height=7em]{pdf/graph_mesh_compile_time_100.pdf}
        \caption{\emph{mesh} - compilation}
        \label{fig:benchmark_results:compile:mesh}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth, height=7em]{pdf/graph_ring_compile_time_100.pdf}
        \caption{\emph{ring} - compilation}
        \label{fig:benchmark_results:compile:ring}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.026\textwidth}
        \includegraphics[width=\textwidth, height=7em]{pdf/time_millisecond.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth, height=7em]{pdf/graph_mesh_runtime_100.pdf}
        \caption{\emph{mesh} - runtime}
        \label{fig:benchmark_results:running:mesh}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth, height=7em]{pdf/graph_ring_runtime_100.pdf}
        \caption{\emph{ring} - runtime}
        \label{fig:benchmark_results:running:ring}
    \end{subfigure}
    \begin{subfigure}[t]{\textwidth}
        \includegraphics[width=\textwidth, height=7em]{pdf/examples.pdf}
    \end{subfigure}
    \caption{
        Microbenchmark results for the \emph{mesh} and \emph{ring} protocols (top)
        and benchmark results for
        Calculator~\cite{hu2016Hybrid} (a),
        Online wallet~\cite{neykova2013Spy} (b),
        SMTP~\cite{postel1982Rfc0821} (c),
        Simple voting~\cite{hu2016Hybrid} (d),
        Three buyers~\cite{jia2016Monitors} (e),
        Travel agency~\cite{huSessionBased2008} (f),
        OAuth~\cite{neykova2013Spy} (g),
        HTTP~\cite{fielding2014Hypertext} (h),
        Remote data \cite{DBLP:journals/sensors/ChenZLCJGYAN22} (i),
        Servo \cite{servoWebEngineBuggy,boquin2020Understanding} (j),
        Gravity sensor \cite{androidMotionSensors} (k),
        PineTime Heart Rate \cite{Pine64} (l),
        and Proximity Based Car Key \cite{propositions2012Wadler,DBLP:journals/pacmpl/IraciandCHZ2023} (m)
        (bottom).
    }
    \Description{
        Microbenchmark results for the mesh and ring protocols (top)
        and benchmark results for
        Calculator~\cite{hu2016Hybrid} (a),
        Online wallet~\cite{neykova2013Spy} (b),
        SMTP~\cite{postel1982Rfc0821} (c),
        Simple voting~\cite{hu2016Hybrid} (d),
        Three buyers~\cite{jia2016Monitors} (e),
        Travel agency~\cite{huSessionBased2008} (f),
        OAuth~\cite{neykova2013Spy} (g),
        HTTP~\cite{fielding2014Hypertext} (h),
        Remote data \cite{DBLP:journals/sensors/ChenZLCJGYAN22} (i),
        Servo \cite{servoWebEngineBuggy,boquin2020Understanding} (j),
        Gravity sensor \cite{androidMotionSensors} (k),
        PineTime Heart Rate \cite{Pine64} (l),
        and Proximity Based Car Key \cite{propositions2012Wadler,DBLP:journals/pacmpl/IraciandCHZ2023} (m)
        (bottom).
    }
    \vspace{-1em}
    \label{fig:benchmark_results_examples}
    \vspace{-1em}
\end{figure}










In addition to the~\emph{mesh} and~\emph{ring} protocols,
we have implemented various examples to showcase the capabilities
of~\timedmulticrusty and conducted benchmarking.
It is important to note that all these examples are originally implemented
in both~\multicrusty and~\timedmulticrusty.
However,
when implemented with~\multicrusty,
these examples lack asynchronous communication and cannot handle timeouts.
The~\CODE{send} and~\CODE{recv} operations are ordered,
directed,
and involve the same participants in both libraries.
On the other hand,
when implemented with~\timedmulticrusty,
these operations are enriched with time constraints and reset predicates.
The benchmark results for the selected examples,
including those from existing literature and two from this paper,
are presented in~\Cref{fig:benchmark_results_examples} (bottom).
To ensure a fair comparison between~\timedmulticrusty
(represented by ${\highlightbox{bordeaux}{\color{bordeaux}bars}}$ bars)
and~\multicrusty (represented by ${\highlightbox{purple}{\color{purple}bars}}$ bars),
time constraints are enforced for all examples without introducing any additional sleep or timeouts.




Apart from the protocols sourced from existing scientific literature,
we have included five additional protocols that use the asynchronous and
timed features of~\timedmulticrusty
extracted from industrial examples.
Besides the Remote Data protocol detailled earlier,
there are three protocol extracted from
\cite{DBLP:journals/pacmpl/IraciandCHZ2023} and one protocol extracted from
\cite{boquin2020Understanding}.
In particular,
the PineTime Heart Rate protocol
\cite{Pine64},
extracted from \cite{DBLP:journals/pacmpl/IraciandCHZ2023}
is a protocol used in the industry
to help the PineTime smartwatch retrieve data from
a heart rate sensor
at a specific pace.






\Cref{fig:benchmark_results_examples} provides a comprehensive
illustration of the capabilities of~\timedmulticrusty,
empowering developers to write,
validate,
and execute communication protocols involving multiple roles,
branching,
and recursion.
Despite additional checks for asynchronous and timed communications,
\timedmulticrusty incurs less than 10\% compilation time and runtime overhead
compared with~\multicrusty.


==> implementation.tex <==









\section{Design and Implementation of \timedmulticrusty}
\label{sec:implementation:implementation}
\label{SEC:IMPLEMENTATION}


In this section,
we provide a detailed description of~\timedmulticrusty,
our~\Rust implementation of \ATMP, inspired by~\multicrusty~\cite{lagaillardie2022Affine}.
\timedmulticrusty has two primary objectives:
correctly cascading failure notifications,
and representing and enforcing time constraints.
To address the first objective,
we use \Rust's native \emph{try-catch} \CODE{?}-operator
in conjunction with optional types.
The approach to the second objective is presented subsequently.
To start, we outline the main challenges encountered during the implementation.




\subparagraph{\bf Challenge 1:  Representation of Time Constraints.}
To handle asynchronous timed communications guided by \ATMP,
we define a time window %
and a corresponding behaviour for each operation.
Implementing this constraint involves addressing two subconstraints:
creating and using clocks in \Rust, and representing
all clock constraints shown in \Cref{sec:session-calculus}.
\Rust enables the creation of virtual clocks that rely on the
CPU's clock and provide accuracy up to the nanosecond level.
Additionally,
the different behaviours can encompass
blocking or non-blocking communications,
pre- or post-specific time tags,
or falling within specified time bounds.
It is crucial to ensure that all these scenarios
are made available to the developer.



\subparagraph{\bf Challenge 2: Enforcement of Time Constraints.}
To effectively enforce time windows,
implementing reliable and accurate clocks and using them correctly
is imperative.
This requires addressing all cases related to time
constraints through appropriate primitives:
clocks may be considered unreliable if they skip ticks,
do not strictly increase,
or if the API for clock comparison does not yield
results quickly enough.
Enforcing time constraints in \timedmulticrusty
is accomplished by using two libraries:
the \crosschan \Rust library~\cite{web:rust:crossbeamChannel},
which our library employs for sending and receiving messages
using asynchronous primitives instead of synchronous ones,
and the \Rust standard library \timeRust \cite{standardTimeLibraryWebsite},
which handles the usage and comparison of virtual clocks.









\input{implementation/implementation/implement_and_enforce_time_bounds.tex}

\input{implementation/implementation/implementation_example_short.tex}


==> introduction_simplified.tex <==
\section{Introduction}
\label{sec:introduction}













\subparagraph*{\bf{Background  \,}}


The increasing prevalence of distributed programming has emphasised the significance
of prioritising~\emph{reliability}
in distributed systems.
A lightweight, type-based methodology, which
ensures basic reliability---\emph{safety}
in distributed communication systems, is
\emph{session types}~\citep{honda1998Language}.
This type discipline is further advanced by
\emph{Multiparty Session Types}~(\MPST)~\cite{honda2008Multiparty},
which enable the specification and verification of communication protocols
among multiple message-passing processes in concurrent and distributed systems.
\MPST ensure that
protocols are designed
to prevent common safety errors,
\ie deadlocks and communication mismatches during interactions among many
participants~(\aka~\emph{end-point programs})~\cite{honda2008Multiparty,DBLP:journals/pacmpl/ScalasY19}. %
From a practical perspective, %
\MPST have been implemented in
various programming
languages~\cite{castro2019Distributed,kouzapas2016Typechecking,
lagaillardie2022Affine,neykova2017timed,viering2021Multiparty,zhouCFSM2021},
facilitating their applications and providing
safety guarantees in
real-world programs.








Nevertheless,
tackling the challenges of unreliability and failures remains
a significant issue for session types.
Most session type systems operate under the assumption of flawless
and reliable communication without failures.
To address this limitation, recent works~\cite{mostrous2018Affine,fowler2019Exceptional,harvey2021Multiparty,lagaillardie2022Affine}
have developed~\emph{affine session types}
 by incorporating the~\emph{affinity} mechanism that explicitly accounts for and handles unreliability
and failures within session type systems.
Unlike linear types that must be used \emph{exactly} once, affine types can be used \emph{at most} once,
enabling the safe dropping of subsequent types and facilitating the premature termination
of a session in the presence of protocol execution errors.



In most real-life devices and platforms, communications are predominantly asynchronous:
inner tasks and message transfers may take time. When dealing with asynchronous communications,
it becomes crucial to incorporate~\emph{time constraints} and implement~\emph{timeout failure handling}
for each operation. This is necessary to avoid potential blockages where a process might wait indefinitely for a message from a non-failed process.
Surprisingly, none of the aforementioned works on affine session types %
explicitly tackles
the challenges of handling specific timeout failures that may occur
during the execution of protocols.


\subparagraph*{\bf{This paper  \,}}  %
introduces a new framework, \emph{affine timed multiparty session types} (\ATMP),
to address the challenges of timeouts, disconnections
and other failures in asynchronous communications:
\begin{enumerate*}
\item We propose \ATMP, an extension of asynchronous \MPST that incorporates time specifications,
affinity, and mechanisms for handling exceptions, thus facilitating effective management of failures, with a particular focus on timeouts.
Additionally, we
demonstrate that properties from~\MPST,
\ie~\emph{type safety}, \emph{protocol conformance},
and~\emph{deadlock-freedom}, are guaranteed for well-typed processes, even
in the presence of timeouts and their corresponding handling mechanism;
\item We present~\timedmulticrusty,
our~\Rust toolchain designed for building asynchronous timed multiparty protocols under~\ATMP:
\timedmulticrusty enables the implementation of protocols adhering to the properties of \ATMP.
\end{enumerate*}




The primary emphasis of our system lies in
effectively~\emph{handling} timeouts during process execution. %
In the context of~\ATMP,
when a process experiences a timeout error,
a mechanism for handling time failures is activated.
This mechanism functions by propagating the notification of
the timeout failure to all participants,
leading to the termination of the notified participants
and the subsequent complete termination of the session.
By employing this mechanism,
we aim to guarantee that participants consistently
reach the~\emph{end of the protocol},
as the communication session is completely terminated
upon encountering a timeout error.
As a result,
every process can successfully terminate,
mitigating the risk of indefinite blockage even in the presence of timeouts.











On the practical side,
we provide~\timedmulticrusty,
a~\Rust implementation of~\ATMP aimed at enabling secure timed communications.
\timedmulticrusty makes use of affine timed meshed channels,
a communication data structure that integrates time constraints and clock utilisation.
Additionally,
we employ affine asynchronous primitives and native optional types
to effectively manage runtime timeouts and errors. %
To showcase the capabilities and expressiveness of our toolchain,
we assess~\timedmulticrusty through examples sourced from existing literature
and additional case studies.
We conduct a comparative analysis of our toolchain
against~\multicrusty, the~\Rust implementation of affine \MPST without time~\cite{lagaillardie2022Affine}, %
revealing that while~\timedmulticrusty exhibits a runtime and compile-time
overhead of less than 10\% compared to~\multicrusty,
it offers significantly stronger property checks.













\subparagraph*{\bf{Paper summary and contributions  \,}}
\textbf{\Cref{sec:overview}} offers a comprehensive overview of our theory and toolchain,
employing the~\emph{Remote Data}
as a running example.
\textbf{\Cref{sec:session-calculus}} provides a session $\pi$-calculus for \ATMP that incorporates timeout, affinity, asynchrony, and failure handling mechanisms.
\textbf{\Cref{sec:aat-mpst-type-system-popl}} presents our extended theory
of asynchronous multiparty session types
with time annotations.
We introduce timed global and local types,
and establish the operational correspondence between them in~\Cref{lem:sound_comp_proj}.
Furthermore,
we present a typing system for~\ATMP session
$\pi$-calculus, and demonstrate type properties
including subject reduction,
session fidelity,
and deadlock-freedom,
in~\Cref{lem:sr_global,lem:aat-mpst-session-fidelity-global,lem:aat-mpst-process-df-proj}. %
\textbf{\Cref{sec:implementation:implementation}} addresses the primary challenges associated
with implementing~\ATMP in~\Rust,
as well as outlining the design and usage of~\timedmulticrusty. %
\textbf{\Cref{sec:evaluation}} depicts the compilation and execution benchmarks of~\timedmulticrusty,
based on selected examples from the literature.
\textbf{\Cref{sec:related_work}} concludes the paper
by discussing related work, and offering potential future work and conclusions. %
\textbf{\emph{Supplemental materials}} (available from HotCRP)
include (1) \textbf{the full version} with
proofs,
detailed definitions, auxiliary material,
and more details of~\timedmulticrusty;
and %
(2) \textbf{\timedmulticrusty}
and its benchmarks. %


==> macros-cfsms.tex <==

\newcommand{\PSEND}[2]{\ptp{#1} ! \msg{#2}}
\newcommand{\PRECEIVE}[2]{\ptp{#1} ? \msg{#2}}
\newcommand{\msg}[1]{\textit{#1}}


\tikzset{
  every state/.style={minimum size=1pt,inner sep=1.2pt, initial text={}},
  mycfsm/.style={
    font=\scriptsize,
    initial where=left,
    initial distance=0.25cm,
    ->,>=stealth,auto, node distance=0.8cm and 0.8cm,
    scale=1, every node/.style={transform shape},
    baseline=(current bounding box.center)
  },
  line/.style = {draw,->, rounded corners=0.07cm,>=latex},
  deliv/.style = {draw, rectangle, rounded corners, fill=white,drop shadow,align=center},
  manip/.style = {draw, ellipse, fill=white,drop shadow,align=center,inner sep=1pt},
  every picture/.style={/utils/exec={\sffamily}}
}



==> macros-mpst.tex <==
\newcommand{\PSet}{\!\mathscr{P}\!}
\newcommand{\ASigma}{ \mathbb{A}}


\newcommand{\ifempty}[3]{%
  \ifthenelse{\isempty{#1}}{#2}{#3}%
}%

\newcommand{\ifTR}[1]{%
  \iftoggle{techreport}{#1}{}%
}%

\newcommand{\dom}[1]{{\color{black}\operatorname{dom}\!\left({#1}\right)}}%
\newcommand{\ran}[1]{{\color{black}\operatorname{ran}\!\left({#1}\right)}}%
\newcommand{\suchthat}{\colon}%
\newcommand{\eqdef}{\colonequals}%
\newcommand{\fn}[1]{\operatorname{fn}\!\left({#1}\right)}%
\newcommand{\sbj}[1]{\operatorname{sbj}\!\left({#1}\right)}%
\newcommand{\bv}[1]{\operatorname{bv}\!\left({#1}\right)}%
\newcommand{\fv}[1]{\operatorname{fv}\!\left({#1}\right)}%
\newcommand{\fc}[1]{\operatorname{fc}\!\left({#1}\right)}%
\newcommand{\dpv}[1]{\operatorname{dpv}\!\left({#1}\right)}%
\newcommand{\fpv}[1]{\operatorname{fpv}\!\left({#1}\right)}%
\newcommand{\sem}[2][]{\mbox{\ensuremath{\llbracket#2\rrbracket_{#1}}}}%
\newcommand{\gfp}[1]{\operatorname{gfp}\!\left({#1}\right)}%
\newcommand{\lfp}[1]{\operatorname{lfp}\!\left({#1}\right)}%
\newcommand{\mfp}[1]{\operatorname{mfp}\!\left({#1}\right)}%
\newcommand{\unfold}[1]{%
  {\color{black}\operatorname{unf^{\ast}}\!\left({#1}\right)}}%
\newcommand{\unfoldOne}[1]{%
  {\color{black}\operatorname{unf}\!\left({#1}\right)}}%
\newcommand{\unfoldN}[2]{%
  {\color{black}\operatorname{unf^{#1}}\!\left({#2}\right)}}%
\newcommand{\notImplies}{\mathrel{{\kern 0.5em}{\not{\kern -0.5em}\implies}}}%
\newcommand{\notImpliedBy}{\mathrel{{\kern 1em}{\not{\kern -1em}\impliedby}}}%
\newcommand{\fix}[1]{\operatorname{fix}\, {#1}}%
\newcommand{\lfix}[1]{\operatorname{lfix}\, {#1}}%

\newcommand{\coloncolonequals}{\Coloneqq}%
\newcommand{\bnfdef}{\coloncolonequals}%
\newcommand{\bnfsep}{\mathbin{\;\big|\;}}%

\def\cf{cf.\@\xspace}%
\def\etc{\emph{etc.}\@\xspace}%
\def\eg{e.g.,\@\xspace}%
\def\Eg{E.g.,\@\xspace}%
\def\ie{i.e.,\@\xspace}%
\def\Ie{I.e.,\@\xspace}%
\def\vs{vs.\@\xspace}%
\def\wrt{w.r.t.\@\xspace}%

\definecolor{ruleColor}{rgb}{0.1, 0.3, 0.1}%
\newcommand{\inferrule}[1]{{\color{ruleColor}\text{\scriptsize [#1]}}}%
\newcommand{\inference}[3][]{\infer[\ifempty{#1}{}{\inferrule{#1}}]{#3}{#2}}%
\newcommand{\cinference}[3][]{\infer=[\ifempty{#1}{}{\inferrule{#1}}]{#3}{#2}}%
\newcommand{\inferenceSingle}[2][]{{#2}\ifempty{#1}{}{\ \inferrule{#1}}}%
\newcommand{\nrule}[1]{{\scriptsize \textsc{#1}}}%

\newcommand{\setenum}[1]{\mathord{{\color{black}\left\{#1\right\}}}}%
\newcommand{\setcomp}[2]{\mathord{%
  {\color{black}\left\{{#1} \,\middle|\, {#2}\right\}}}}%
\newcommand{\card}[1]{\mathord{\left\vert{#1}\right\vert}}

\newcommand{\setenumSmall}[1]{\mathord{{\color{black}\{#1\}}}}%
\newcommand{\setcompSmall}[2]{\mathord{{\color{black}\{{#1} \,\mid\, {#2}\}}}}%
\newcommand{\cardSmall}[1]{\mathord{\vert{#1}\vert}}%

\newcommand{\setNat}{\mathord{\mathbb{N}}}%
\newcommand{\setNatZero}{\mathord{\mathbb{N}^0}}%
\newcommand\someSetX{\mathord{\mathbb{X}}}%
\newcommand\someSetY{\mathord{\mathbb{Y}}}%

\newcommand{\setLabelTypes}{\mathbb{L}}%

\definecolor{groundColor}{rgb}{0.38, 0.25, 0.32}%

\newcommand{\groundFmt}[1]{{\color{groundColor}#1}}%
\newcommand{\setGroundTypes}{\groundFmt{\mathbb{B}}}%
\newcommand{\groundSubtype}{\mathrel{\groundFmt{\leqslant_{\setGroundTypes}}}}%

\newcommand{\someDeriv}[1][]{\ifempty{#1}{\mathcal{D}}{\mathcal{D}_{#1}}}%

\newcommand{\bind}[2]{\nicefrac{#2}{#1}}
\newcommand{\substenum}[1]{\mathord{{\color{black}\left\{{#1}\right\}}}}
\newcommand{\subst}[2]{\substenum{\bind{#1}{#2}}}
\newcommand{\mapsubst}[2]{{#1}{\mapsto}{#2}}

\definecolor{roleColor}{rgb}{0.5, 0.0, 0.0}%
\newcommand{\roleCol}[1]{{\color{roleColor}#1}}%
\newcommand{\roleUnivSet}{\roleCol{\mathfrak{R}}}%
\newcommand{\roleSet}{\roleCol{\mathbb{R}}}%
\newcommand{\roleFmt}[1]{\boldsymbol{\roleCol{\mathtt{#1}}}}%
\newcommand{\roleP}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{p}}}{{\color{roleColor}\roleFmt{p}_{{#1}}}}%
}%
\newcommand{\rolePi}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{p}'}}{{\color{roleColor}\roleFmt{p}'_{#1}}}%
}%
\newcommand{\roleQ}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{q}}}{{\color{roleColor}\roleFmt{q}_{#1}}}%
}%
\newcommand{\roleQi}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{q}'}}{{\color{roleColor}\roleFmt{q}'_{#1}}}%
}%
\newcommand{\roleR}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{r}}}{{\color{roleColor}\roleFmt{r}_{\!#1}}}%
}%
\newcommand{\roleRi}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{r}'}}{{\color{roleColor}\roleFmt{r}'_{\!#1}}}%
}%
\newcommand{\roleRii}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{r}''}}{{\color{roleColor}\roleFmt{r}''_{\!#1}}}%
}%

\newcommand{\labFmt}[2][]{\color{roleColor}{\ifempty{#1}{\mathtt{#2}}{\mathtt{#2}\textsubscript{#1}}}}%

\definecolor{mpColor}{rgb}{0, 0, 0}%
\newcommand{\mpFmt}[1]{{\color{mpColor}#1}}%

\newcommand{\mpLab}[1][]{%
  \mpFmt{\ifempty{#1}{\labFmt{m}}{{\labFmt{m}}_{\mathnormal #1}}}%
}%

\newcommand{\mpRequest}[1][]{%
  \mpFmt{\ifempty{#1}{\labFmt{req}}{{\labFmt{req}}_{\mathnormal #1}}}%
}%

\newcommand{\mpResponse}[1][]{%
\mpFmt{\ifempty{#1}{\labFmt{res}}{{\labFmt{res}}_{\mathnormal #1}}}%
}%

\newcommand{\mpVideo}[1][]{%
\mpFmt{\ifempty{#1}{\labFmt{video}}{{\labFmt{video}}_{\mathnormal #1}}}%
}%

\newcommand{\mpClose}[1][]{%
\mpFmt{\ifempty{#1}{\labFmt{close}}{{\labFmt{close}}_{\mathnormal #1}}}%
}%

\newcommand{\mpQuestion}{{\color{blue}{\textbf{?}}}\,}%
\newcommand{\mpDagger}{\roleFmt{\dagger}\,}%

\newcommand{\mpLabi}[1][]{%
  \mpFmt{\ifempty{#1}{\labFmt{m}'}{\labFmt{m}'_{\mathnormal #1}}}%
}%
\newcommand{\mpLabFmt}[1]{\mpFmt{\labFmt{#1}}}%

\newcommand{\proclit}[1]{\ensuremath{\operatorname{\text{\sffamily\bfseries{#1}}}}}

\newcommand{\mpTrue}{\mpFmt{\text{\emph{\texttt{true}}}}}%
\newcommand{\mpFalse}{\mpFmt{\text{\emph{\texttt{false}}}}}%
\newcommand{\mpString}[1]{\text{\emph{\texttt{"{#1}"}}}}%

\newcommand{\mpChanRole}[2]{\mpFmt{{#1}[{#2}]}}%
\newcommand{\mpChanRoles}[3]{\mpFmt{{#1}[{#2}][{#3}]}}%



\newcommand{\mpNil}{\mpFmt{\mathbf{0}}}%
\newcommand{\mpSeq}{\mathbin{\mpFmt{\!.\!}}}%
\newcommand{\mpExpr}{\mpFmt{e}}%
\newcommand{\EvalExpr}{\downarrow}%

\newcommand{\mpIf}[3]{%
  \mpFmt{\proclit{if}\,{#1}\,\proclit{then}}\,{#2}\,\proclit{else}\,{#3}%
}%
\newcommand{\mpChoice}[3]{%
  \mpFmt{%
    \mpLabFmt{#1}\ifempty{#2}{}{({#2})}\ifempty{#3}{}{\vphantom{x}\mpSeq {#3}}%
  }%
}%
\newcommand{\mpChoiceNoBind}[3]{%
  \mpFmt{%
    \mpLabFmt{#1}\ifempty{#2}{}{\langle{#2}\rangle}\ifempty{#3}{}{\vphantom{x}\mpSeq {#3}}%
  }%
}%
\newcommand{\mpBranchRaw}[3]{%
  \mpFmt{%
    {#1}[\roleFmt{#2}] \sum%
      {#3}%
  }%
}%
\newcommand{\mpBranch}[6]{%
\mpFmt{%
  {#1}[\roleFmt{#2}] \mathbin{\!\ifempty{\sum}{\&}{\sum_{#3}}\!}%
  \ifempty{#3}{%
    \mpChoice{#4}{#5}{#6}%
  }{%
    \mpChoice{#4}{#5}{#6}%
  }%
}%
}%
\newcommand{\mpBranchSeq}[5]{%
\mpFmt{%
  {#1}[\roleFmt{#2}]\mpChoice{#3}{#4}{#5}%
}%
}%
\newcommand{\mpBranchSolo}[4]{%
\mpFmt{%
  {#1} \mpChoice{#2}{#3}{#4}%
}%
}%
\newcommand{\mpQuestionBranch}[6]{%
\mpFmt{%
  \mpQuestion{#1}[\roleFmt{#2}] \mathbin{\!\ifempty{\sum}{\&}{\sum_{#3}}\!}%
  \ifempty{#3}{%
    \mpChoice{#4}{#5}{#6}%
  }{%
    \mpChoice{#4}{#5}{#6}%
  }%
}%
}%
\newcommand{\mpQuestionBranchSeq}[5]{%
\mpFmt{%
  \mpQuestion{#1}[\roleFmt{#2}]\mpChoice{#3}{#4}{#5}%
}%
}%
\newcommand{\mpQuestionBranchSolo}[3]{%
\mpFmt{%
  \mpQuestion{#1}[\roleFmt{#2}]\mpFmt{({#3})}%
}%
}%
\newcommand{\mpDaggerBranch}[6]{%
  \mpFmt{%
    \mpDagger{#1}[\roleFmt{#2}] \mathbin{\!\ifempty{\sum}{\&}{\sum_{#3}}\!}%
    \ifempty{#3}{%
      \mpChoice{#4}{#5}{#6}%
    }{%
      \mpChoice{#4}{#5}{#6}%
    }%
  }%
}%

\newcommand{\mpQuestionSel}[5]{%
  \mpFmt{%
    \mpQuestion{#1}[\roleFmt{#2}] \mathbin{\!\oplus\!}%
    \mpChoiceNoBind{#3}{#4}{#5}%
  }%
}%

\newcommand{\mpDaggerSel}[5]{%
  \mpFmt{%
    \mpDagger{#1}[\roleFmt{#2}] \mathbin{\!\oplus\!}%
    \mpChoiceNoBind{#3}{#4}{#5}%
  }%
}%
\newcommand{\mpSel}[5]{%
  \mpFmt{%
    {#1}[\roleFmt{#2}] \mathbin{\!\oplus\!}%
    \mpChoiceNoBind{#3}{#4}{#5}%
  }%
}%


\newcommand{\mpRaise}[2]{\chanraise(#1).{#2}}%
\newcommand{\mpPar}{\mathbin{\mpFmt{\mid}}}%
\newcommand{\mpParTall}{\mathbin{\mpFmt{\bigm|}}}%
\newcommand{\mpBigPar}[2]{\mathbin{\mpFmt{\Pi_{#1}}{#2}}}%
\newcommand{\mpRes}[2]{\mpFmt{\left(\mathbf{\nu}{#1}\right){#2}}}%
\newcommand{\mpRec}[2]{\mpFmt{\mu{#1}.{#2}}}%
\newcommand{\mpJustDef}[3]{%
  \mpFmt{{#1}(#2) = {#3}}%
}%
\newcommand{\mpDef}[4]{%
  \mpFmt{\proclit{def}\;\mpJustDef{#1}{#2}{#3}\;\proclit{in}\;{#4}}%
}%
\newcommand{\mpDefAbbrev}[2]{%
  \mpFmt{\proclit{def}\;{#1}\;\proclit{in}\;{#2}}%
}%
\newcommand{\mpAngleDef}[3]{%
\mpFmt{{#1}\langle#2\rangle = {#3}}%
}%
\newcommand{\mpShortAngleDef}[3]{%
\mpFmt{\proclit{def}\;\mpAngleDef{#1}{#2}{#3}}%
}%
\newcommand{\mpCall}[2]{\mpFmt{{#1}\!\left\langle{#2}\right\rangle}}%
\newcommand{\mpErr}{\mpFmt{\boldsymbol{\mathsf{err}}}}%
\newcommand{\mpRaiseProc}{\mpFmt{\proclit{raise}}}%


\newcommand{\mpCtx}[1][]{\mpFmt{\ifempty{#1}{\mathbb{C}}{\mathbb{C}_{#1}}}}%
\newcommand{\mpEtx}[1][]{\mpFmt{\ifempty{#1}{\mathbb{E}}{\mathbb{E}_{#1}}}}%
\newcommand{\mpCtxi}[1][]{\mpFmt{\ifempty{#1}{\mathbb{C}'}{\mathbb{C}'_{#1}}}}%
\newcommand{\mpCtxii}[1][]{\mpFmt{\ifempty{#1}{\mathbb{C}''}{\mathbb{C}''_{#1}}}}%
\newcommand{\mpCtxHole}{[\,]}%
\newcommand{\mpEtxHole}{[\,]}%
\newcommand{\mpCtxApp}[2]{{#1}\!\left[{#2}\right]}%

\newcommand{\mpA}[1][]{\mpFmt{\ifempty{#1}{a}{a_{#1}}}}%
\newcommand{\mpAi}[1][]{\mpFmt{\ifempty{#1}{a'}{a'_{#1}}}}%
\newcommand{\mpAii}[1][]{\mpFmt{\ifempty{#1}{a''}{a''_{#1}}}}%

\newcommand{\mpC}[1][]{\mpFmt{\ifempty{#1}{c}{c_{#1}}}}%
\newcommand{\mpCi}[1][]{\mpFmt{\ifempty{#1}{c'}{c'_{#1}}}}%
\newcommand{\mpCii}[1][]{\mpFmt{\ifempty{#1}{c''}{c''_{#1}}}}%
\newcommand{\mpD}[1][]{\mpFmt{\ifempty{#1}{d}{d_{#1}}}}%
\newcommand{\mpConst}{\mathtt{d}}%

\newcommand{\mpDi}[1][]{\mpFmt{\ifempty{#1}{d'}{d'_{#1}}}}%
\newcommand{\mpDii}[1][]{\mpFmt{\ifempty{#1}{d''}{d''_{#1}}}}%

\newcommand{\mpS}[1][]{\mpFmt{\ifempty{#1}{s}{s_{#1}}}}%
\newcommand{\mpSi}[1][]{\mpFmt{\ifempty{#1}{s'}{s'_{#1}}}}%
\newcommand{\mpSii}[1][]{\mpFmt{\ifempty{#1}{s''}{s''_{#1}}}}%
\newcommand{\mpSiii}[1][]{\mpFmt{\ifempty{#1}{s'''}{s'''_{#1}}}}%

\newcommand{\mpX}[1][]{\mpFmt{\ifempty{#1}{X}{X_{#1}}}}%
\newcommand{\mpXi}[1][]{\mpFmt{\ifempty{#1}{X'}{X'_{#1}}}}%
\newcommand{\mpY}[1][]{\mpFmt{\ifempty{#1}{Y}{Y_{#1}}}}%
\newcommand{\mpZ}[1][]{\mpFmt{\ifempty{#1}{Z}{Z_{#1}}}}%
\newcommand{\mpZi}[1][]{\mpFmt{\ifempty{#1}{Z'}{Z'_{#1}}}}%
\newcommand{\mpZii}[1][]{\mpFmt{\ifempty{#1}{Z''}{Z''_{#1}}}}%

\newcommand{\mpP}[1][]{\mpFmt{\ifempty{#1}{P}{P_{#1}}}}%
\newcommand{\mpPi}[1][]{\mpFmt{\ifempty{#1}{P'}{P'_{#1}}}}%
\newcommand{\mpPii}[1][]{\mpFmt{\ifempty{#1}{P''}{P''_{#1}}}}%
\newcommand{\mpPiii}[1][]{\mpFmt{\ifempty{#1}{P'''}{P'''_{#1}}}}%
\newcommand{\mpPx}[1][]{\mpFmt{\ifempty{#1}{P^\bullet}{P^\bullet_{#1}}}}%
\newcommand{\mpQ}[1][]{\mpFmt{\ifempty{#1}{Q}{Q_{#1}}}}%
\newcommand{\mpQi}[1][]{\mpFmt{\ifempty{#1}{Q'}{Q'_{#1}}}}%
\newcommand{\mpQii}[1][]{\mpFmt{\ifempty{#1}{Q''}{Q''_{#1}}}}%
\newcommand{\mpR}[1][]{\mpFmt{\ifempty{#1}{R}{R_{#1}}}}%
\newcommand{\mpRi}[1][]{\mpFmt{\ifempty{#1}{R'}{R'_{#1}}}}%
\newcommand{\mpRii}[1][]{\mpFmt{\ifempty{#1}{R''}{R''_{#1}}}}%

\newcommand{\mpT}[1][]{\mpFmt{\ifempty{#1}{T}{T_{#1}}}}%

\newcommand{\mpDefD}[1][]{\mpFmt{\ifempty{#1}{D}{D_{#1}}}}%
\newcommand{\mpDefDi}[1][]{\mpFmt{\ifempty{#1}{D'}{D'_{#1}}}}%
\newcommand{\mpDefDii}[1][]{\mpFmt{\ifempty{#1}{D''}{D''_{#1}}}}%

\newcommand{\mpMove}{\to}%
\newcommand{\mpMoveAnnot}[4]{\xrightarrow{\mpAnnot{#1}{#2}{#3}{#4}}}%
\newcommand{\mpMoveAnnotDef}{\xrightarrow{\mpFmt{\proclit{def}}}}%
\newcommand{\mpMoveAnnotDefStar}{\mathrel{\mpMoveAnnotDef{}^{\!\!\!\!*}}}%
\newcommand{\mpAnnot}[4]{{#1}{[#2]}{[#3]}{#4}}%
\newcommand{\mpMoveStar}{\mathrel{\mpMove{}^{\!\!\!*}}}%
\newcommand{\mpMoveP}[1]{\mpFmt{#1}\!{\mpMove}}%
\newcommand{\mpNotMoveP}[1]{\mpFmt{#1}\!\not\!\!{\mpMove}}%

\definecolor{gtColor}{rgb}{0.43, 0.21, 0.1}%
\newcommand{\gtFmt}[1]{{\color{gtColor}#1}}%
\newcommand{\gtMsgFmt}[1]{\gtFmt{\labFmt{#1}}}%
\newcommand{\gtLab}[1][]{%
  \ifempty{#1}{\gtMsgFmt{m}}{{\color{gtColor}\gtMsgFmt{m}_{#1}}}%
}%
\newcommand{\gtLabi}[1][]{%
  \ifempty{#1}{\gtMsgFmt{m}'}{{\color{gtColor}\gtMsgFmt{m}'_{#1}}}%
}%

\newcommand{\gtG}[1][]{\gtFmt{\ifempty{#1}{G}{G_{#1}}}}%
\newcommand{\gtGi}[1][]{\gtFmt{\ifempty{#1}{G'}{G'_{#1}}}}%
\newcommand{\gtGii}[1][]{\gtFmt{\ifempty{#1}{G''}{G''_{#1}}}}%
\newcommand{\gtGiii}[1][]{\gtFmt{\ifempty{#1}{G'''}{G'''_{#1}}}}%

\newcommand{\gtSeq}{\mathbin{\gtFmt{.}}}%

\newcommand{\gtCommRaw}[3]{%
  \gtFmt{%
    {#1} {\to} {#2}{:}%
    \left\{%
      {#3}%
    \right\}%
  }%
}%
\newcommand{\gtComm}[6]{%
  \gtFmt{%
    \gtCommRaw{#1}{#2}{%
      \gtCommChoice{#4}{#5}{#6}%
    }_{#3}%
  }%
}%
\newcommand{\gtCommSingle}[5]{%
  \gtFmt{%
    {#1} {\to} {#2}{:}%
    \gtCommChoice{#3}{#4}{#5}%
  }%
}%
\newcommand{\gtCommChoice}[3]{%
  \gtFmt{%
    \gtMsgFmt{#1}\ifempty{#2}{}{({#2})}%
    \ifempty{#3}{}{\vphantom{x}{\gtSeq}{#3}}%
  }%
}%
\newcommand{\gtCommChoiceSmall}[3]{%
  \gtFmt{%
    \gtMsgFmt{#1}\ifempty{#2}{}{({#2})}%
    \ifempty{#3}{}{\vphantom{x} \!\gtSeq\! {#3}}%
  }%
}%

\newcommand{\gtEnd}{\gtFmt{\mathbf{end}}}%

\newcommand{\gtRec}[2]{\gtFmt{\mu{#1}.{#2}}}%
\newcommand{\gtRecVarBase}{\gtFmt{\mathbf{t}}}%
\newcommand{\gtRecVar}[1][]{\gtFmt{\ifempty{#1}{\gtRecVarBase}{\gtRecVarBase_{#1}}}}%
\newcommand{\gtRecVari}[1][]{\gtFmt{\ifempty{#1}{\gtRecVarBase'}{\gtRecVarBase'_{#1}}}}%
\newcommand{\gtRecVarii}[1][]{\gtFmt{\ifempty{#1}{\gtRecVarBase'}{\gtRecVarBase'_{#1}}}}

\newcommand{\gtRoles}[1]{{\color{black} \operatorname{roles}(\gtFmt{#1})}}%

\newcommand{\gtProj}[2]{%
  {\color{stColor}\gtFmt{#1} {\upharpoonright} #2}%
}%

\newcommand{\gtCtx}[1][]{\gtFmt{\ifempty{#1}{\mathbb{G}}{\mathbb{G}_{#1}}}}%
\newcommand{\gtCtxi}[1][]{\gtFmt{\ifempty{#1}{\mathbb{G}'}{\mathbb{G}'_{#1}}}}%
\newcommand{\gtCtxHole}[1]{\gtFmt{[\;]^{#1}}}%
\newcommand{\gtCtxApp}[4]{\gtFmt{{#1}[{#2}]^{#3}_{#4}}}%

\definecolor{stColor}{rgb}{0.1, 0.4, 0.1}%
\newcommand{\stFmt}[1]{{\color{stColor}#1}}%

\newcommand{\stTypeBool}{\stFmt{\operatorname{Bool}}}%
\newcommand{\stTypeInt}{\stFmt{\operatorname{Int}}}%
\newcommand{\stTypeString}{\stFmt{\operatorname{Str}}}%

\newcommand{\stInTag}{?}%
\newcommand{\stOutTag}{!}%
\newcommand{\stIn}[3]{\ifempty{#1}{}{\roleFmt{#1}}\stFmt{\&{#2}\ifempty{#3}{}{({#3})}}}%
\newcommand{\stOut}[3]{\ifempty{#1}{}{\roleFmt{#1}}\stFmt{\oplus{#2}\ifempty{#3}{}{({#3})}}}%

\newcommand{\stChoice}[2]{\stFmt{#1}\ifempty{#2}{}{\stFmt{({#2})}}}%

\newcommand{\stTau}{\stFmt{\tau}}%
\newcommand{\stSeq}{\mathbin{\!\stFmt{.}\!}}%
\newcommand{\stIntC}{\mathbin{\stFmt{\oplus}}}%
\newcommand{\stIntSum}[3]{\roleFmt{#1}\stFmt{\oplus_{#2}{#3}}}%





\newcommand{\stExtC}{\mathbin{\stFmt{\&}}}%
\newcommand{\stExtSum}[3]{\roleFmt{#1}\stFmt{\&_{#2}{#3}}}%
\newcommand{\stGenSum}[3]{\roleFmt{#1}\stFmt{\maltese_{#2}{#3}}}%
\newcommand{\stGenC}{\mathbin{\stFmt{\maltese}}}%
\newcommand{\stGenSumDual}[3]{\roleFmt{#1}\,\stFmt{\bar{\maltese}_{#2}{#3}}}%
\newcommand{\stRec}[2]{\stFmt{\mu{#1}.{#2}}}%
\newcommand{\stEnd}{\stFmt{\mathbf{end}}}%

\newcommand{\stLab}[1][]{\mpFmt{\ifempty{#1}{\labFmt{m}}{\labFmt{m}_{#1}}}}%
\newcommand{\stLabi}[1][]{\mpFmt{\ifempty{#1}{\labFmt{m}'}{\labFmt{m}'_{#1}}}}%
\newcommand{\stLabFmt}[1]{\mpFmt{\labFmt{#1}}}%

\newcommand{\stS}[1][]{\stFmt{\ifempty{#1}{S}{S_{#1}}}}%
\newcommand{\stSi}[1][]{\stFmt{\ifempty{#1}{S'}{S'_{#1}}}}%
\newcommand{\stSii}[1][]{\stFmt{\ifempty{#1}{S''}{S''_{#1}}}}%
\newcommand{\stSiii}[1][]{\stFmt{\ifempty{#1}{S'''}{S'''_{#1}}}}%
\newcommand{\stSiiii}[1][]{\stFmt{\ifempty{#1}{S''''}{S''''_{#1}}}}%

\newcommand{\stT}[1][]{\stFmt{\ifempty{#1}{T}{T_{#1}}}}%
\newcommand{\stTi}[1][]{\stFmt{\ifempty{#1}{T'}{T'_{#1}}}}%
\newcommand{\stTii}[1][]{\stFmt{\ifempty{#1}{T''}{T''_{#1}}}}%
\newcommand{\stTiii}[1][]{\stFmt{\ifempty{#1}{T'''}{T'''_{#1}}}}%

\newcommand{\stU}[1][]{\stFmt{\ifempty{#1}{U}{U_{#1}}}}%
\newcommand{\stUi}[1][]{\stFmt{\ifempty{#1}{U'}{U'_{#1}}}}%
\newcommand{\stUii}[1][]{\stFmt{\ifempty{#1}{U''}{U''_{#1}}}}%
\newcommand{\stUiii}[1][]{\stFmt{\ifempty{#1}{U'''}{U'''_{#1}}}}%

\newcommand{\stLabP}[1][]{\stFmt{\stLab[#1](\stS[#1])}}%
\newcommand{\stLabPi}[1][]{\stFmt{\stLabi[#1](\stSi[#1])}}%

\newcommand{\stRecVarBase}{\stFmt{\mathbf{t}}}%
\newcommand{\stRecVar}[1][]{\stFmt{\ifempty{#1}{\stRecVarBase}{\stRecVarBase_{#1}}}}%
\newcommand{\stRecVari}[1][]{\stFmt{\ifempty{#1}{\stRecVar'}{\stRecVar'_{#1}}}}%
\newcommand{\stRecVarii}[1][]{\stFmt{\ifempty{#1}{\stRecVar''}{\stRecVar''_{#1}}}}%

\newcommand{\stRoles}[1]{\stFmt{#1}}%
\newcommand{\stRolesSet}[1]{\operatorname{roles}(\stFmt{#1})}%

\newcommand{\stCtx}[1][]{\stFmt{\ifempty{#1}{\mathbb{S}}{\mathbb{S}_{#1}}}}%
\newcommand{\stCtxi}[1][]{\stFmt{\ifempty{#1}{\mathbb{S}'}{\mathbb{S}'_{#1}}}}%
\newcommand{\stCtxHole}[1]{\stFmt{[\;]^{#1}}}%
\newcommand{\stCtxApp}[4]{\stFmt{{#1}[{#2}]^{#3}_{#4}}}%

\newcommand{\stMerge}[2]{\stFmt{\bigsqcap_{#1}{#2}}}%
\newcommand{\stBinMerge}{\mathbin{\stFmt{\sqcap}}}%

\newcommand{\stProj}[2]{%
  {\color{ptColor}\stFmt{#1} {\upharpoonright} \roleFmt{#2}}%
}%

\newcommand{\stSub}{\mathrel{\stFmt{\leqslant}}}%
\newcommand{\stNotSub}{\mathrel{\stFmt{\not\leqslant}}}%
\newcommand{\stSup}{\mathrel{\stFmt{\geqslant}}}%
\newcommand{\stEquiv}{\mathrel{\stFmt{\equiv}}}%

\definecolor{ptColor}{rgb}{0.20, 0.29, 0.09}%
\newcommand{\ptFmt}[1]{{\color{ptColor}#1}}%

\newcommand{\ptInTag}{?}%
\newcommand{\ptOutTag}{!}%
\newcommand{\ptIn}[2]{\ptFmt{\&{#1}\ifempty{#2}{}{({#2})}}}%
\newcommand{\ptOut}[2]{\ptFmt{\oplus{#1}\ifempty{#2}{}{({#2})}}}%

\newcommand{\ptChoice}[2]{\ptFmt{#1}\ifempty{#2}{}{\ptFmt{({#2})}}}%

\newcommand{\ptSeq}{\mathbin{\!\ptFmt{.}\!}}%
\newcommand{\ptIntC}{\mathbin{\ptFmt{\oplus}}}%
\newcommand{\ptIntSum}[2]{\ptFmt{\oplus_{#1}{#2}}}%
\newcommand{\ptExtC}{\mathbin{\ptFmt{\&}}}%
\newcommand{\ptExtSum}[2]{\ptFmt{\&_{#1}{#2}}}%
\newcommand{\ptGenSum}[2]{\ptFmt{\Large{\maltese}_{#1}{#2}}}%
\newcommand{\ptRec}[2]{\ptFmt{\mu{#1}.{#2}}}%
\newcommand{\ptEnd}{\ptFmt{\mathbf{end}}}%

\newcommand{\ptLab}[1][]{\ptFmt{\ifempty{#1}{\labFmt{m}}{\labFmt{m}_{#1}}}}%
\newcommand{\ptLabFmt}[1]{\ptFmt{\labFmt{#1}}}%

\newcommand{\ptH}[1][]{\ptFmt{\ifempty{#1}{H}{H_{#1}}}}%
\newcommand{\ptHi}[1][]{\ptFmt{\ifempty{#1}{H'}{H'_{#1}}}}%
\newcommand{\ptHii}[1][]{\ptFmt{\ifempty{#1}{H''}{H''_{#1}}}}%
\newcommand{\ptHiii}[1][]{\ptFmt{\ifempty{#1}{H'''}{H'''_{#1}}}}%

\newcommand{\ptRecVar}{\ptFmt{\mathbf{t}}}%
\newcommand{\ptRecVari}[1][]{\ptFmt{\ifempty{#1}{\ptRecVar'}{\ptRecVar'_{#1}}}}%
\newcommand{\ptRecVarii}[1][]{\ptFmt{\ifempty{#1}{\ptRecVar'}{\ptRecVar'_{#1}}}}

\newcommand{\ptMerge}[2]{\ptFmt{\bigsqcap_{#1}{#2}}}%
\newcommand{\ptBinMerge}{\mathbin{\ptFmt{\sqcap}}}%

\newcommand{\ptDual}[1]{\ptFmt{\overline{#1}}}%

\newcommand{\ptSub}{\mathrel{\ptFmt{\leqslant}}}%
\newcommand{\ptNotSub}{\mathrel{\ptFmt{\not\leqslant}}}%
\newcommand{\ptSup}{\mathrel{\ptFmt{\geqslant}}}%

\newcommand{\ptQPfx}[2]{\ptFmt{\stFmt{#1}{\bullet}\ptFmt{#2}}}%

\newcommand{\stEnv}[1][]{\stFmt{\ifempty{#1}{\Gamma}{\Gamma_{#1}}}}%
\newcommand{\stEnvi}[1][]{\stFmt{\ifempty{#1}{\Gamma'}{\Gamma'_{#1}}}}%
\newcommand{\stEnvii}[1][]{\stFmt{\ifempty{#1}{\Gamma''}{\Gamma''_{#1}}}}%
\newcommand{\stEnviii}[1][]{\stFmt{\ifempty{#1}{\Gamma'''}{\Gamma'''_{#1}}}}%
\newcommand{\stEnvEmpty}{\stFmt{\emptyset}}%
\newcommand{\stEnvMap}[2]{\stFmt{\mpFmt{#1}\mathbin{\!:\!}{#2}}}%
\newcommand{\stEnvMapBig}[2]{\stFmt{\mpFmt{#1}\mathbin{:}{#2}}}%
\newcommand{\stEnvComp}{\mathpunct{\stFmt{,}}}%
\newcommand{\stEnvApp}[2]{\stFmt{#1\!\left(\mpFmt{#2}\right)}}%

\newcommand{\stEnvMove}{\mathrel{\stFmt{\to}}}%
\newcommand{\stEnvAnnotOutSym}{\stFmt{\oplus}}%
\newcommand{\stEnvAnnotInSym}{\stFmt{\&}}%
\newcommand{\stEnvAnnotTauSym}{\stFmt{,}}%
\newcommand{\stEnvAnnotGenericSym}{\stFmt{\alpha}}%
\newcommand{\stEnvMoveAnnot}[1]{\mathrel{\stFmt{\xrightarrow{#1}}}}
\newcommand{\stEnvMoveGenAnnot}{\stEnvMoveAnnot{\stEnvAnnotGenericSym}}%
\newcommand{\stEnvMoveInAnnot}[3]{%
  \stEnvMoveAnnot{\stEnvInAnnot{#1}{#2}{#3}}%
}%
\newcommand{\stEnvMoveOutAnnot}[3]{%
  \stEnvMoveAnnot{\stEnvOutAnnot{#1}{#2}{#3}}%
}%
\newcommand{\stEnvMoveCommAnnot}[3]{%
  \stEnvMoveAnnot{\stEnvCommAnnot{#1}{#2}{#3}}%
}%
\newcommand{\stEnvInAnnot}[3]{\stFmt{\mpS:{#1}{\stEnvAnnotInSym}{#2}:{#3}}}%
\newcommand{\stEnvOutAnnot}[3]{\stFmt{\mpS:{#1}{\stEnvAnnotOutSym}{#2}:{#3}}}%
\newcommand{\stEnvCommAnnot}[3]{\stFmt{\mpS:{#1}{\stEnvAnnotTauSym}{#2}:{#3}}}%
\newcommand{\stEnvInAnnotSmall}[3]{\mpS{:}\stFmt{{#1}{\stEnvAnnotInSym}{#2}{:}{#3}}}%
\newcommand{\stEnvOutAnnotSmall}[3]{\stFmt{\mpS{:}{#1}{\stEnvAnnotOutSym}{#2}{:}{#3}}}%
\newcommand{\stEnvCommAnnotSmall}[3]{\stFmt{\mpS{:}{#1}{\stEnvAnnotTauSym}{#2}{:}{#3}}}%
\newcommand{\stEnvCommAnnotSmalli}[3]{\stFmt{\mpSi{:}{#1}{\stEnvAnnotTauSym}{#2}{:}{#3}}}%
\newcommand{\stEnvMoveP}[1]{{#1}\!\!\stEnvMove}%
\newcommand{\stEnvNotMoveP}[1]{{#1}\!\!\not\stEnvMove}%
\newcommand{\stEnvMoveStar}{\mathrel{\stFmt{\stEnvMove{}^{\!\!\!*}}}}%
\newcommand{\stEnvMoveAnnotP}[2]{{#1}\!\!\stEnvMoveAnnot{#2}}%
\newcommand{\stEnvMoveGenAnnotP}[1]{{#1}\!\!\stEnvMoveGenAnnot}%
\newcommand{\stEnvNotMoveGenAnnotP}[1]{{#1}\!\!\not\stEnvMoveGenAnnot}%

\newcommand{\stEnvBeh}[1]{\operatorname{beh}(\stFmt{#1})}%
\newcommand{\stEnvQBeh}[2]{\operatorname{a-beh_{{#1}}}(\stFmt{#2})}%

\newcommand{\stEnvEndPred}{\operatorname{end}}%
\newcommand{\stEnvEndP}[1]{\stEnvEndPred(\stFmt{#1})}%

\newcommand{\stEnvTermPred}{\operatorname{term}}%
\newcommand{\stEnvTermP}[1]{\stEnvTermPred(\stFmt{#1})}%

\newcommand{\stEnvNeverTermPred}{\operatorname{nterm}}%
\newcommand{\stEnvNeverTermP}[1]{\stEnvNeverTermPred(\stFmt{#1})}%

\newcommand{\stEnvDFPred}{\operatorname{df}}%
\newcommand{\stEnvDFP}[1]{\stEnvDFPred(\stFmt{#1})}%

\newcommand{\stEnvLivePred}{\operatorname{live}}%
\newcommand{\stEnvLiveP}[1]{\stEnvLivePred(\stFmt{#1})}%
\newcommand{\stEnvNotLiveP}[1]{\neg\stEnvLivePred(\stFmt{#1})}%

\newcommand{\stEnvKLivePred}[1][k]{\operatorname{live_{\text{${#1}$}}}}%
\newcommand{\stEnvKLiveP}[2][k]{\stEnvKLivePred[{#1}](\stFmt{#2})}%
\newcommand{\stEnvNotKLiveP}[2][k]{\neg\stEnvKLivePred[{#1}](\stFmt{#2})}%

\newcommand{\stEnvLivePlusPred}{\operatorname{live^{+}}}%
\newcommand{\stEnvLivePlusP}[1]{\stEnvLivePlusPred(\stFmt{#1})}%
\newcommand{\stEnvNotLivePlusP}[1]{\neg\stEnvLivePlusPred(\stFmt{#1})}%

\newcommand{\stEnvLivePlusPlusPred}{\operatorname{live^{++}}}%
\newcommand{\stEnvLivePlusPlusP}[1]{\stEnvLivePlusPlusPred(\stFmt{#1})}%
\newcommand{\stEnvNotLivePlusPlusP}[1]{\neg\stEnvLivePlusPlusPred(\stFmt{#1})}%

\newcommand{\stEnvSafePred}{\operatorname{safe}}%
\newcommand{\stEnvSafeP}[1]{\stEnvSafePred(\stFmt{#1})}%
\newcommand{\stEnvNotSafeP}[1]{\neg\stEnvSafePred(\stFmt{#1})}%

\newcommand{\stEnvProjPred}[2]{\operatorname{fproj_{{#1},{#2}}}}%
\newcommand{\stEnvProjP}[3]{\stEnvProjPred{#1}{#2}(\stFmt{#3})}%
\newcommand{\stEnvNotProjP}[3]{\neg\stEnvProjPred{#1}{#2}(\stFmt{#3})}%

\newcommand{\stEnvProjPlainPred}[2]{\operatorname{pproj}_{{#1},{#2}}}%
\newcommand{\stEnvProjPlainP}[3]{\stEnvProjPlainPred{#1}{#2}(\stFmt{#3})}%
\newcommand{\stEnvNotProjPlainP}[3]{\neg\stEnvProjPredPlain{#1}{#2}(\stFmt{#3})}%

\newcommand{\stEnvConsistentPred}{\operatorname{consistent}}%
\newcommand{\stEnvConsistentP}[1]{\stEnvConsistentPred(\stFmt{#1})}%
\newcommand{\stEnvNotConsistentP}[1]{\neg\stEnvConsistentPred(\stFmt{#1})}%

\newcommand{\stEnvEntails}[3]{%
  \stFmt{#1} \vdash \stFmt{\mpFmt{#2} \mathbin{\!:\!} {#3}}%
}%
\newcommand{\stEnvDel}[2]{%
  \stFmt{{#1} \mathbin{\!{\backslash}\!} {\color{black}{#2}}}%
}%

\newcommand{\mpEnv}[1][]{\stFmt{\ifempty{#1}{\Theta}{\Theta_{#1}}}}%
\newcommand{\mpEnvi}[1][]{\stFmt{\ifempty{#1}{\Theta'}{\Theta'_{#1}}}}%
\newcommand{\mpEnvii}[1][]{\stFmt{\ifempty{#1}{\Theta''}{\Theta''_{#1}}}}%
\newcommand{\mpEnvEmpty}{\stFmt{\emptyset}}%
\newcommand{\mpEnvMap}[2]{\stFmt{\mpFmt{#1}{:}\stFmt{#2}}}%
\newcommand{\mpEnvMapBig}[3]{\stFmt{\stFmt{#1}:\stEnvGR{#2}{#3}}}%
\newcommand{\mpEnvComp}{\mathpunct{\stFmt{,}}}%
\newcommand{\mpEnvApp}[2]{\stFmt{#1}\!\left(\mpFmt{#2}\right)}%

\newcommand{\mpEnvEntails}[3]{%
  \stFmt{#1} \vdash \stFmt{\mpFmt{#2} \mathbin{\!:\!} \stFmt{#3}}%
}%

\newcommand{\stJudge}[3]{%
  \stFmt{\ifempty{#1}{#2}{{#1} \cdot {#2}}%
  \mathrel{\mpFmt{\vdash}} \mpFmt{#3}}%
}%

\newcommand{\stJudgeTry}[3]{%
 \stFmt{\ifempty{#1}{#2}{{#1} \cdot {#2}}%
 \mathrel{\mpFmt{\vDash}} \mpFmt{#3}}%
}%
\newcommand{\stJudgeSplit}[3]{%
  \stFmt{\ifempty{#1}{#2}{%
    \begin{array}{@{\hskip 0mm}r@{\hskip 0mm}}
    {#1}%
    \\%
    \vphantom{x} \cdot%
    {#2}%
    \end{array}
  }%
  \mathrel{\mpFmt{\vdash}} \mpFmt{#3}}%
}%
\newcommand{\stJudgeInit}[3]{%
  \stFmt{\ifempty{#1}{#2}{{#1} \cdot {#2}}%
  \mathrel{\mpFmt{\vdash_{\rm init}}} \mpFmt{#3}}%
}%

\newcommand{\mpSessionStack}[2]{%
  \mpFmt{{#1}\mathrel{\!\blacktriangleright\!}{#2}}}%
\newcommand{\mpStack}[1][]{\mpFmt{\ifempty{#1}{\sigma}{\sigma_{#1}}}}%
\newcommand{\mpStacki}[1][]{\mpFmt{\ifempty{#1}{\sigma'}{\sigma'_{#1}}}}%
\newcommand{\mpStackii}[1][]{\mpFmt{\ifempty{#1}{\sigma''}{\sigma''_{#1}}}}%
\newcommand{\mpStackiii}[1][]{\mpFmt{\ifempty{#1}{\sigma'''}{\sigma'''_{#1}}}}%
\newcommand{\mpStackEmpty}{\mpFmt{\epsilon}}%
\newcommand{\mpStackElem}[4]{%
  \mpFmt{\left({#1},{#2},{#3}\ifempty{#4}{}{\langle{#4}\rangle}\right)}}%
\newcommand{\mpStackCons}[2]{\mpFmt{{#1}\mathrel{\!\cdot\!}{#2}}}%

\newcommand{\mpStackSenders}[1]{\operatorname{senders}\!\left({#1}\right)}%

\newcommand{\stEnvQ}[1][]{\stFmt{\ifempty{#1}{\Gamma}{\Gamma_{#1}}}}%
\newcommand{\stEnvQi}[1][]{\stFmt{\ifempty{#1}{\Gamma'}{\Gamma'_{#1}}}}%
\newcommand{\stEnvQii}[1][]{\stFmt{\ifempty{#1}{\Gamma''}{\Gamma''_{#1}}}}%
\newcommand{\stEnvQiii}[1][]{\stFmt{\ifempty{#1}{\Gamma'''}{\Gamma'''_{#1}}}}%
\newcommand{\stEnvQComp}{\mathpunct{\stFmt{,}}}%
\newcommand{\stEnvQCompStack}{\stFmt{\leftsquigarrow}}%
\newcommand{\stEnvQCompStackAppend}{\stFmt{\rightsquigarrow}}%
\newcommand{\stEnvQEmpty}{\stFmt{\emptyset}}%
\newcommand{\stQJudge}[4]{%
  \stFmt{\ifempty{#1}{#2}{{#1} \cdot {#2}}%
  \mathrel{\mpFmt{\vdash}_{\mpFmt{#3}}} \mpFmt{#4}}%
}%

\newcommand{\stEnvQAnnotStackSym}{\stFmt{!}}%
\newcommand{\stEnvQAnnotRecvSym}{\stFmt{,}}%
\newcommand{\stEnvQStackAnnot}[3]{\stFmt{\mpS:{#1}{\stEnvQAnnotStackSym}{#2}:{#3}}}%
\newcommand{\stEnvQRecvAnnot}[3]{\stFmt{\mpS:{#1}{\stEnvQAnnotRecvSym}{#2}:{#3}}}%
\newcommand{\stEnvQStackAnnotSmall}[3]{\stFmt{\mpS{:}{#1}{\stEnvQAnnotStackSym}{#2}{:}{#3}}}%
\newcommand{\stEnvQRecvAnnotSmall}[3]{\stFmt{\mpS{:}{#1}{\stEnvQAnnotRecvSym}{#2}{:}{#3}}}%
\newcommand{\stEnvQMoveAnnot}[1]{\mathrel{\stFmt{\xrightarrow{#1}}}}
\newcommand{\stEnvQMoveGenAnnot}{\stEnvMoveAnnot{\stEnvAnnotGenericSym}}%
\newcommand{\stEnvQMoveStackAnnot}[3]{%
  \stEnvQMoveAnnot{\stEnvQStackAnnotSmall{#1}{#2}{#3}}%
}%
\newcommand{\stEnvQMoveRecvAnnot}[3]{%
  \stEnvQMoveAnnot{\stEnvQRecvAnnotSmall{#1}{#2}{#3}}%
}%

\newcommand{\mpSessionSet}[1][]{%
  \mpFmt{\ifempty{#1}{\mathcal{S}}{\mathcal{S}_{#1}}}}%
\newcommand{\mpSessionSeti}[1][]{%
  \mpFmt{\ifempty{#1}{\mathcal{S}'}{\mathcal{S}'_{#1}}}}%

\newcommand{\stQ}[1][]{\stFmt{\ifempty{#1}{M}{M_{#1}}}}%
\newcommand{\stQi}[1][]{\stFmt{\ifempty{#1}{M'}{M'_{#1}}}}%
\newcommand{\stQii}[1][]{\stFmt{\ifempty{#1}{M''}{M''_{#1}}}}%
\newcommand{\stQEmpty}{\stFmt{\epsilon}}%
\newcommand{\stQCons}[2]{\stFmt{{#1}\mathbin{\!\cdot\!}{#2}}}%
\newcommand{\stQMsg}[3]{\stFmt{{#1}\mathbin{\!\mathbf{!}\!}{#2}\ifempty{#3}{}{({#3})}}}%
\newcommand{\stQMsgWide}[3]{\stFmt{{#1}\mathbin{\mathbf{!}}{#2}\ifempty{#3}{}{({#3})}}}%
\newcommand{\stQProj}[2]{\stFmt{{#1}(\roleFmt{#2})}}%

\newcommand{\stQEquiv}{\mathrel{\stFmt{\equiv}}}%

\newcommand{\stM}[1][]{\stFmt{\ifempty{#1}{\tau}{\tau_{#1}}}}%
\newcommand{\stMi}[1][]{\stFmt{\ifempty{#1}{\tau'}{\tau'_{#1}}}}%
\newcommand{\stMii}[1][]{\stFmt{\ifempty{#1}{\tau''}{\tau''_{#1}}}}%
\newcommand{\stMPair}[2]{\stFmt{({#2}{\mathbin{\mathbf{;\,}}}{#1})}}%

\newcommand{\stEnvQMove}{\mathrel{\stFmt{\to}}}%
\newcommand{\stEnvQMoveStar}{\mathrel{\stEnvQMove{}^{\!\!\!*}}}%
\newcommand{\stEnvQMoveP}[1]{{#1}\!\!\stEnvQMove}%
\newcommand{\stEnvQNotMoveP}[1]{{#1}\!\!\not\stEnvQMove}%
\newcommand{\stEnvQMoveModQ}[1]{\mathrel{\stFmt{\rightarrow}_{{#1}}}}%
\newcommand{\stEnvQMoveAnnotModQ}[2]{%
  \mathrel{\stFmt{\xrightarrow{#1}}_{{#2}}}%
}%
\newcommand{\stEnvQMoveGenAnnotModQ}[1]{%
  \stEnvQMoveAnnotModQ{\stEnvAnnotGenericSym}{#1}%
}%
\newcommand{\stEnvQMoveStackAnnotModQ}[4]{%
  \stEnvQMoveAnnotModQ{\stEnvQStackAnnot{#2}{#3}{#4}}{#1}%
}%
\newcommand{\stEnvQMoveRecvAnnotModQ}[4]{%
  \stEnvQMoveAnnotModQ{\stEnvQRecvAnnot{#2}{#3}{#4}}{#1}%
}%
\newcommand{\stEnvQMoveGenAnnotModQP}[2]{{#1}\!\!\stEnvQMoveGenAnnotModQ{#2}}%
\newcommand{\stEnvQNotMoveGenAnnotModQP}[2]{{#1}\!\!\not\stEnvQMoveGenAnnotModQ{#2}}%
\newcommand{\stEnvQMoveAnnotModQP}[3]{{#1}\!\!\stEnvQMoveAnnotModQ{#2}{#3}}%

\newcommand{\stEnvQMoveModQStar}[1]{%
  \mathrel{\stEnvQMoveModQ{{#1}}^{\!\!\!*}}}%
\newcommand{\stEnvQMoveModQP}[2]{{#2}\!\!\stEnvQMoveModQ{#1}}%
\newcommand{\stEnvQNotMoveModQP}[2]{%
  {#2}/{\kern -0.5em}{\stEnvQMoveModQ{#1}}}%

\newcommand{\stEnvQBMove}[1][]{%
  \ifempty{#1}{%
    \mathrel{\to_{\!(b)}}%
  }{%
    \mathrel{\to_{\!({#1})}}%
  }%
}%

\newcommand{\stEnvQEndPred}[1]{\operatorname{a-end_{#1}}}%
\newcommand{\stEnvQEndP}[2]{\stEnvQEndPred{#1}({#2})}%
\newcommand{\stEnvQDFPred}[1]{\operatorname{a-df_{#1}}}%
\newcommand{\stEnvQDFP}[2]{\stEnvQDFPred{#1}({#2})}%
\newcommand{\stEnvQTermPred}[1]{\operatorname{a-term_{#1}}}%
\newcommand{\stEnvQTermP}[2]{\stEnvQTermPred{#1}({#2})}%
\newcommand{\stEnvQNeverTermPred}[1]{\operatorname{a-nterm_{#1}}}%
\newcommand{\stEnvQNeverTermP}[2]{\stEnvQNeverTermPred{#1}({#2})}%
\newcommand{\stEnvQSafePred}[1]{\operatorname{a-safe_{#1}}}%
\newcommand{\stEnvQSafeP}[2]{\stEnvQSafePred{#1}(\stFmt{#2})}%
\newcommand{\stEnvQNotSafeP}[2]{\neg\stEnvQSafePred{#1}(\stFmt{#2})}%
\newcommand{\stEnvQConsistentPred}[1]{\operatorname{a-consistent_{#1}}}%
\newcommand{\stEnvQConsistentP}[2]{\stEnvQConsistentPred{#1}({#2})}%
\newcommand{\stEnvQLivePred}[1]{\operatorname{a-live_{#1}}}%
\newcommand{\stEnvQLiveP}[2]{\stEnvQLivePred{#1}({#2})}%

\newcommand{\stEnvQKLivePred}[2][k]{\operatorname{a-live_{\text{${#1}-{#2}$}}}}%
\newcommand{\stEnvQKLiveP}[3][k]{\stEnvQKLivePred[{#1}]{#2}(\stFmt{#3})}%
\newcommand{\stEnvQNotKLiveP}[3][k]{\neg\stEnvQKLivePred[{#1}]{#2}(\stFmt{#3})}%

\newcommand{\stEnvQLivePlusPred}[1]{\operatorname{a-live^{+}_{#1}}}%
\newcommand{\stEnvQLivePlusP}[2]{\stEnvQLivePlusPred{#1}(\stFmt{#2})}%
\newcommand{\stEnvQNotLivePlusP}[2]{\neg\stEnvQLivePlusPred{#1}(\stFmt{#1})}%

\newcommand{\stEnvQLivePlusPlusPred}[1]{\operatorname{a-live^{++}_{#1}}}%
\newcommand{\stEnvQLivePlusPlusP}[2]{\stEnvQLivePlusPlusPred{#1}(\stFmt{#2})}%
\newcommand{\stEnvQNotLivePlusPlusP}[2]{\neg\stEnvQLivePlusPlusPred{#1}(\stFmt{#1})}%

\newcommand{\stEnvQLiveKBoundedPred}[2][k]{\operatorname{a-live_{\text{${#2}$}}-bound_{\text{${#1}$}}}}%
\newcommand{\stEnvQLiveKBoundedP}[3][k]{\stEnvQLiveKBoundedPred[{#1}]{#2}(\stFmt{#3})}%
\newcommand{\stEnvQNotLiveKBoundedP}[3][k]{\neg\stEnvQLiveKBoundedPred[{#1}]{#2}(\stFmt{#3})}%

\newcommand{\stEnvQLiveBoundedPred}[1]{\operatorname{a-live_{\text{${#1}$}}-bound}}%
\newcommand{\stEnvQLiveBoundedP}[2]{\stEnvQLiveBoundedPred{#1}(\stFmt{#2})}%
\newcommand{\stEnvQNotLiveBoundedP}[2]{\neg\stEnvQLiveBoundedPred{#1}(\stFmt{#1})}%

\newcommand{\stEnvQKBoundedPred}[2][k]{\operatorname{a-bound_{\text{${#2}$,${#1}$}}}}%
\newcommand{\stEnvQKBoundedP}[3][k]{\stEnvQKBoundedPred[{#1}]{#2}(\stFmt{#3})}%
\newcommand{\stEnvQNotKBoundedP}[3][k]{\neg\stEnvQKBoundedPred[{#1}]{#2}(\stFmt{#3})}%

\newcommand{\stEnvQBoundedPred}[1]{\operatorname{a-bound_{{#1}}}}%
\newcommand{\stEnvQBoundedP}[2]{\stEnvQBoundedPred{#1}(\stFmt{#2})}%
\newcommand{\stEnvQNotBoundedP}[2]{\neg\stEnvQBoundedPred{#1}(\stFmt{#1})}%


\newcommand{\predP}[1][]{\ifempty{#1}{\varphi}{\varphi_{#1}}}%
\newcommand{\predPi}[1][]{\ifempty{#1}{\varphi'}{\varphi'_{#1}}}%
\newcommand{\predPii}[1][]{\ifempty{#1}{\varphi''}{\varphi''_{#1}}}%
\newcommand{\predPApp}[2][]{\ifempty{#1}{\predP}{\predP[{#1}]}\!\left({#2}\right)}%

\newcommand{\relC}{\mathrel{\mathcal{C}}}%
\newcommand{\relD}{\mathrel{\mathcal{D}}}%
\newcommand{\relDi}{\mathrel{\mathcal{D}_1}}%
\newcommand{\relDii}{\mathrel{\mathcal{D}_2}}%
\newcommand{\relR}[1][]{\mathrel{\ifempty{#1}{\mathcal{R}}{\mathcal{R}_{#1}}}}%
\newcommand{\relRi}[1][]{\mathrel{\ifempty{#1}{\mathcal{R}'}{\mathcal{R}'_{#1}}}}%
\newcommand{\relRii}[1][]{\mathrel{\ifempty{#1}{\mathcal{R}''}{\mathcal{R}''_{#1}}}}%

\newcommand{\bisim}{\sim}%
\newcommand{\wbisim}{\approx}%

\newcommand{\OKmark}{{\color{Green}\text{\ding{51}}}}%
\newcommand{\KOmark}{{\color{Red}\text{\ding{55}}}}%

\newcommand{\muCol}[1]{{\color{red}#1}}%
\newcommand{\muFmt}[1]{\muCol{\mathsf{#1}}}%

\newcommand{\muJudge}[2]{{#1} \mathrel{\muCol{\models}} \muCol{#2}}%
\newcommand{\muJudgeNeg}[2]{{#1} \mathrel{\muCol{\not\models}} {#2}}%

\newcommand{\muVar}[1][]{\muCol{\ifempty{#1}{\muFmt{Z}}{\muFmt{Z}_{#1}}}}%
\newcommand{\muVari}[1][]{\muCol{\ifempty{#1}{\muFmt{Z}'}{\muFmt{Z}'_{#1}}}}%

\newcommand{\muData}[1][]{\muCol{\ifempty{#1}{\muFmt{d}}{\muFmt{d}_{#1}}}}%

\newcommand{\muAct}[1][]{\muCol{\ifempty{#1}{\alpha}{\alpha_{#1}}}}%

\newcommand{\muStar}[1]{\mathord{{#1}^{\muCol{*}}}}%
\newcommand{\muOmega}[1]{\mathord{{#1}^{\muCol{\omega}}}}%
\newcommand{\muInf}[1]{\mathord{{#1}^{\muCol{\infty}}}}%

\newcommand{\muActSet}{\muCol{\mathbb{A}\mathrm{ct}}}%
\newcommand{\muActSetStar}{\muStar{\muActSet}}%
\newcommand{\muActSetOmega}{\muOmega{\muActSet}}%
\newcommand{\muActSetInf}{\muInf{\muActSet}}%

\newcommand{\muSomeActSet}[1][]{\muCol{\ifempty{#1}{\mathbb{A}}{\mathbb{A}_{#1}}}}%

\newcommand{\muForall}[2]{\muCol{\forall{#1}\mathbin{\!.\!}{#2}}}%
\newcommand{\muExists}[2]{\muCol{\exists{#1}\mathbin{\!.\!}{#2}}}%
\newcommand{\muNotExists}[2]{\muCol{\not\exists{#1}\mathbin{\!.\!}{#2}}}%

\newcommand{\muPred}[1][]{\muCol{\ifempty{#1}{\phi}{\phi_{#1}}}}%
\newcommand{\muPredi}[1][]{\muCol{\ifempty{#1}{\phi'}{\phi'_{#1}}}}%
\newcommand{\muPredii}[1][]{\muCol{\ifempty{#1}{\phi''}{\phi''_{#1}}}}%

\newcommand{\muNeg}[1]{\muCol{\neg{#1}}}%
\newcommand{\muAnd}{\mathbin{\muCol{\land}}}%
\newcommand{\muBigAnd}[2]{\muCol{\bigwedge_{#1}{#2}}}%
\newcommand{\muPrefix}[2]{\muCol{({#1}){#2}}}%
\newcommand{\muBox}[2]{\muCol{[{#1}]{#2}}}%
\newcommand{\muDiamond}[2]{\muCol{\langle{#1}\rangle{#2}}}%
\newcommand{\muTrue}{\muCol{\top}}%
\newcommand{\muGFP}[2]{\muCol{\nu{#1}\mathbin{\!.\!}{#2}}}%

\newcommand{\muLFP}[2]{\muCol{\mu{#1}\mathbin{\!.\!}{#2}}}%
\newcommand{\muOr}{\mathbin{\muCol{\lor}}}%
\newcommand{\muBigOr}[2]{\muCol{\bigvee_{#1}{#2}}}%
\newcommand{\muFalse}{\muCol{\bot}}%
\newcommand{\muImplies}{\mathbin{\muCol{\Rightarrow}}}%
\newcommand{\muPrefixNeg}[2]{\muCol{(-{#1}){#2}}}%

\newcommand{\muAlways}[1]{\muCol{\square{#1}}}%
\newcommand{\muEventually}[1]{\muCol{\lozenge{#1}}}%
\newcommand{\muUntil}[2]{\muCol{{#1} \mathbin{\muFmt{U}} {#2}}}%

\newcommand{\muVal}[1][]{%
  \muCol{\ifempty{#1}{\mathcal{V}}{\mathcal{V}_{#1}}}
}%
\newcommand{\muVali}[1][]{%
  \muCol{\ifempty{#1}{\mathcal{V}'}{\mathcal{V}'_{#1}}}
}%
\newcommand{\muValApp}[2]{\muCol{{#1}\!\left({#2}\right)}}%
\newcommand{\muValUpdate}[3]{\muCol{{#1}\!\subst{#2}{#3}}}%
\newcommand{\muDenot}[2]{\muCol{\left\lVert{#1}\right\rVert_{#2}}}%

\newcommand{\muWord}[1][]{\muCol{\ifempty{#1}{\sigma}{\sigma_{#1}}}}%
\newcommand{\muWordEmpty}[1][]{\muCol{\epsilon}}%
\newcommand{\muWordHead}[1]{\muCol{\operatorname{\muFmt{hd}}\!\left({#1}\right)}}%
\newcommand{\muWordTail}[1]{\muCol{\operatorname{\muFmt{tl}}\!\left({#1}\right)}}%
\newcommand{\muWordSet}{\muCol{\mathbb{W}}}%

\newcommand{\iruleMPRedComm}{R-Com}%
\newcommand{\iruleMPQuestionRedComm}{R-?Com}%
\newcommand{\iruleMPPromote}{T-$\vDash$}%
\newcommand{\iruleMPRedSt}{R-Struct}%
\newcommand{\iruleMPRedPar}{R-$\mpPar$}%
\newcommand{\iruleMPRedRes}{R-$\mpFmt{\mathbf{\nu}}$}%
\newcommand{\iruleMPRedDef}{R-$\mpFmt{\mathbf{def}}$}%
\newcommand{\iruleMPRedCall}{R-Def}%
\newcommand{\iruleMPRedCongr}{R-$\equiv$}%
\newcommand{\iruleMPRedCtx}{R-Ctx}%
\newcommand{\iruleMPRedCat}{R-Cat}%
\newcommand{\iruleMPRedCan}{R-Can}%
\newcommand{\iruleMPCSel}{C-Sel}%
\newcommand{\iruleMPCQSel}{C-?Sel}%
\newcommand{\iruleMPTQSel}{T?Sel}%
\newcommand{\iruleMPTQBra}{T?Br}%
\newcommand{\iruleMPCQBra}{C-?Br}%
\newcommand{\iruleMPCBra}{C-Br}%
\newcommand{\iruleMPCCat}{C-Cat}%
\newcommand{\iruleMPTCat}{TCat}%

\newcommand{\iruleTCtxOut}{$\stEnv$-$\stFmt{\oplus}$}%
\newcommand{\iruleTCtxIn}{$\stEnv$-$\stFmt{\&}$}%
\newcommand{\iruleTCtxCom}{$\stEnv$-Comm}%
\newcommand{\iruleTCtxRec}{$\stEnv$-$\mu$}%
\newcommand{\iruleTCtxCong}{$\stEnv$-Cong}%

\newcommand{\iruleATCtxCom}{$\stEnv$-AComm}%
\newcommand{\iruleATCtxMsg}{$\stEnv$-AMsg}%

\newcommand{\iruleDTCtxCom}{$\stEnv$-DCom}%
\newcommand{\iruleDSTCtxMsg}{$\stEnv$-DMsg}%
\newcommand{\iruleDTCtxBase}{$\stEnv$-Base}%

\newcommand{\iruleMPErrLabel}{R-Err}%
\newcommand{\iruleMPTimeOutLabel}{R-TOut}%


\newcommand{\iruleMPRedOutA}{R-AOut}%
\newcommand{\iruleMPRedInA}{R-AIn}%
\newcommand{\iruleMPErrLabelA}{R-AErr}%

\newcommand{\iruleSubEnd}{Sub-$\stEnd$}%
\newcommand{\iruleSubBranch}{Sub-$\stExtC$}%
\newcommand{\iruleSubSel}{Sub-$\stIntC$}%
\newcommand{\iruleSubRecL}{Sub-$\stFmt{\mu}$L}%
\newcommand{\iruleSubRecR}{Sub-$\stFmt{\mu}$R}%

\newcommand{\irulePTSubEnd}{PTSub-$\stEnd$}%
\newcommand{\irulePTSubBranch}{PTSub-$\stExtC$}%
\newcommand{\irulePTSubSel}{PTSub-$\stIntC$}%
\newcommand{\irulePTSubRecL}{PTSub-$\stFmt{\mu}$L}%
\newcommand{\irulePTSubRecR}{PTSub-$\stFmt{\mu}$R}%

\newcommand{\iruleMPEnd}{T-$\stEnvEndPred$}%
\newcommand{\iruleMPX}{T-$\mpFmt{X}$}%
\newcommand{\iruleMPSub}{T-sub}%
\newcommand{\iruleMPRaise}{T-raise}%
\newcommand{\iruleMPNarrow}{T-Narrow}%
\newcommand{\iruleMPNil}{T-$\mpNil$}%
\newcommand{\iruleMPDef}{T-def}%
\newcommand{\iruleMPDefTry}{T-def-try}%
\newcommand{\iruleMPCall}{T-call}%
\newcommand{\iruleMPCallTry}{T-$\mpX$-Try}%
\newcommand{\iruleMPCancel}{T-cancel}%
\newcommand{\iruleMPSusp}{Susp}%
\newcommand{\iruleMPKills}{T-kill}%
\newcommand{\iruleMPTryCatch}{T-try}%
\newcommand{\iruleMPTryCatchInit}{T-try-init}%
\newcommand{\iruleMPErr}{T-err}%
\newcommand{\iruleMPOp}{T-Op}%
\newcommand{\iruleMPPar}{T-$\mpPar$}%
\newcommand{\iruleMPResProp}{T-$\mpFmt{\mathbf{\nu}}$}%
\newcommand{\iruleMPRes}{T-$\mpFmt{\mathbf{\nu}}$Classic}%
\newcommand{\iruleMPSafeRes}{T-$\mpFmt{\mathbf{\nu}}$}%
\newcommand{\iruleMPGenRes}{TGen-$\mpFmt{\mathbf{\nu}}$}%
\newcommand{\iruleMPBranch}{T-$\mpFmt{\&}$}%
\newcommand{\iruleMPQSel}{T-$\mpQuestion\mpFmt{\oplus}$}%
\newcommand{\iruleMPQBranch}{T-$\mpQuestion\mpFmt{\&}$}%
\newcommand{\iruleMPSel}{T-$\mpFmt{\oplus}$}%
\newcommand{\iruleMPInit}{T-init}%

\newcommand{\iruleSafeComm}{S-${\stIntC}{\stExtC}$}%
\newcommand{\iruleSafeRec}{S-$\stFmt{\mu}$}%
\newcommand{\iruleSafeMove}{S-$\stEnvMove$}%

\newcommand{\iruleMPLiftA}{TA-Lift}%
\newcommand{\iruleMPParA}{TA-$\mpPar$}%
\newcommand{\iruleMPResAProp}{TA-$\mpFmt{\mathbf{\nu}}$}%
\newcommand{\iruleMPResA}{TA-$\mpFmt{\mathbf{\nu}}$Classic}%
\newcommand{\iruleMPGenResA}{TAGen-$\mpFmt{\mathbf{\nu}}$}%
\newcommand{\iruleMPStackEmptyA}{TA-$\mpStackEmpty$}%
\newcommand{\iruleMPStackA}{TA-$\mpStack$}%

\newcommand{\iruleSafeQComm}{SA-${\stExtC}{\stFmt{!}}$}%
\newcommand{\iruleSafeQExtQ}{SA-${\stExtC}{\stQ}$}%
\newcommand{\iruleSafeQRec}{SA-$\stFmt{\mu}$}%
\newcommand{\iruleSafeQMove}{SA-$\stEnvMove$}%

\newcommand{\iruleLiveBranch}{L-$\stFmt{\&}$}%
\newcommand{\iruleLiveSel}{L-$\stFmt{\oplus}$}%
\newcommand{\iruleLiveRec}{L-$\stFmt{\mu}$}%
\newcommand{\iruleLiveMove}{L-$\stEnvMove$}%

\newcommand{\iruleLivePlusBranch}{L-$\stFmt{\&}^+$}%
\newcommand{\iruleLivePlusSel}{L-$\stFmt{\oplus}^+$}%
\newcommand{\iruleLivePlusRec}{L-$\stFmt{\mu}^+$}%
\newcommand{\iruleLivePlusMove}{L-$\stEnvMove^+$}%
\newcommand{\iruleLivePlusPlusBranch}{L-$\stFmt{\&}^{++}$}%
\newcommand{\iruleLivePlusPlusSel}{L-$\stFmt{\oplus}^{++}$}%

\newcommand{\iruleLiveQBranch}{LA-$\stFmt{\&}$}%
\newcommand{\iruleLiveQOut}{LA-$\stFmt{!}$}%
\newcommand{\iruleLiveQRec}{LA-$\stFmt{\mu}$}%
\newcommand{\iruleLiveQMove}{LA-$\stEnvQMoveModQ{\!}$}%

\newcommand{\iruleLivePQBranch}{LA-$\stFmt{\&}^+$}%
\newcommand{\iruleLivePQOut}{LA-$\stFmt{!}^+$}%

\newcommand{\iruleLivePPQBranch}{LA-$\stFmt{\&}^{++}$}%
\newcommand{\iruleLivePPQOut}{LA-$\stFmt{!}^{++}$}%

\newcommand{\iruleKLiveBranch}{L$k$-$\stFmt{\&}$}%
\newcommand{\iruleKLiveSel}{L$k$-$\stFmt{\oplus}$}%

\newcommand{\iruleKLiveQBranch}{LA$k$-$\stFmt{\&}$}%
\newcommand{\iruleKLiveQOut}{LA$k$-$\stFmt{!}$}%

\newcommand{\iruleTravSetTarget}{TS-Target}%
\newcommand{\iruleTravSetComm}{TS-Comm}%

\newcommand{\iruleTravSetTargetAsync}{TSA-Target}%
\newcommand{\iruleTravSetIOAsync}{TS-IO}%
\newcommand{\AMPST}{{\sf{AMPST}}\xspace}%
\newcommand{\MPST}{{\sf{MPST}}\xspace}%
\newcommand{\BST}{{\sf{BST}}\xspace}%

\newcommand{\kills}[1]{\ensuremath{{#1} \lightning}}

\newcommand{\mpCancel}[2]{\ifempty{#1}{}{\proclit{cancel}({#1})}{\ifempty{#2}{}{.{#2}}}}
\newcommand{\trycatch}[2]{\ensuremath{\proclit{try}\ {#1} \ \proclit{catch}\ {#2}}}
\newcommand{\trycatchbreakequal}[3]{
  \ensuremath{
    \begin{array}{@{}l@{}}
      {#1} = \proclit{try}\ {#2}
    } \\ \qquad \qquad \ensuremath{\proclit{catch}\ {#3}}
  \end{array}
}
\newcommand{\trycatchbreak}[2]{
  \ensuremath{
    \begin{array}{@{}l@{}}
      \proclit{try}\ {#1}
    } \\ \qquad \ensuremath{\proclit{catch}\ {#2}}
  \end{array}
}


\definecolor{ColourGlobal}{rgb}{.816,.125,.565} %
\definecolor{ColourLocal}{rgb}{0,0,.5} %
\definecolor{ColourLabel}{rgb}{.5,0,.5} %
\definecolor{ColourParticipant}{rgb}{0,.5,.5} %
\definecolor{Blue}{rgb}{0,0,1} %
\definecolor{ColourShade}{rgb}{0.94, 1.0, 0.96} %
\definecolor{Yellow}{rgb}{1,1,0}

\newcommand{\roleAlice}{{\color{roleColor}\roleFmt{A}}}%
\newcommand{\roleBob}{{\color{roleColor}\roleFmt{B}}}%
\newcommand{\roleCarol}{{\color{roleColor}\roleFmt{C}}}%

\newcommand{\chanraise}{{\color{roleColor}\proclit{err}}}%



==> protocol_mesh.tex <==


\begin{tikzpicture}[
    role/.style={circle,text width=2em,text centered,draw,inner sep=0,font=\small},
    arrow/.style={>=latex,thick,draw},
    label/.style={inner sep=2,font=\sf\small},
    transform shape,
    scale = 0.7
  ]
  \node (p0)[role] {A};
  \node (p1) [role,below=of p0] {B}
    edge [arrow,<-] node [label,midway,fill=white] {ping} (p0)
    edge [arrow,->,bend left=45] node [label,midway,left] {pong} (p0);
  \node (c) [role,right=2 of p1] {C}
    edge [bend right=20,arrow,->] node [label,midway,fill=white] {ping} (p0)
    edge [arrow,<-] node [label,midway,fill=white] {pong} (p0)
    edge [bend left=10,arrow,->] node [label,midway,fill=white] {ping} (p1)
    edge [bend right=10,arrow,<-] node [label,midway,fill=white] {pong} (p1);
\end{tikzpicture}





==> protocol_ring.tex <==


\begin{tikzpicture}[
    role/.style={circle,text width=2em,text centered,draw,inner sep=0,font=\small},
    arrow/.style={>=latex,thick,draw},
    label/.style={inner sep=3,font=\sf\small},
    transform shape,
    scale = 0.7
]
\node (p0) [role] {$\text{\normalfont A}_\text{\normalfont 1}$};
\node (p1) [role,right=of p0] {$\text{\normalfont A}_\text{\normalfont 2}$}
edge [bend left=30,arrow,->] node [midway,below,label]{pong} (p0)
edge [bend right=30,arrow,<-] node [midway,above,label]{ping}(p0);
\node (p2) [role,right=of p1] {$\text{\normalfont A}_\text{\normalfont 3}$}
edge [bend left=30,arrow,->] node [midway,below,label]{pong} (p1)
edge [bend right=30,arrow,<-] node [midway,above,label]{ping}(p1);
\node (p3) [role,right=of p2] {$\text{\normalfont A}_\text{\normalfont n}$}
edge [densely dashed,bend left=30,arrow,->] node [midway,below,label]{pong} (p2)
edge [densely dashed,bend right=30,arrow,<-] node [midway,above,label]{ping}(p2);
\end{tikzpicture}


==> typingsystem/gt-lts.tex <==
\begin{figure}[t]
\[
\small
\begin{array}{c}
\begin{array}{c}
 \highlight{ \inferenceSingle[\iruleGtMoveTime]{
    \gtWithTime{\cVal}{\gtG}
    \gtMove[\timeLab]
    \gtWithTime{\cVal + \timeLab}{\gtG}
  }}
\end{array}
\qquad
\begin{array}{c}
  \inference[\iruleGtMoveRec]{
    \gtWithTime{\cVal}{\gtG{}\subst{\gtRecVar}{\gtRec{\gtRecVar}{\gtG}}}
    \gtMove[\stEnvAnnotGenericSym]
    \gtWithTime{\cVali}{\gtGi}}
  {
    \gtWithTime{\cVal}{\gtRec{\gtRecVar}{\gtG}}
    \gtMove[\stEnvAnnotGenericSym]
    \gtWithTime{\cVali}{\gtGi}
  }
  \end{array}
  \\[2ex]

  \inference[\iruleGtMoveOut]{
    j \in I
    &
   \highlight{ \cVal \models \ccstO[j]}
    &
   \highlight{\cVali = \cValUpd{\cVal}{\crstO[j]}{0}}
  }{
    \gtWithTime{\cVal}{
      \gtCommTSmall{\roleP}{\roleQ}{i \in I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtGi[i]}
    }
    \gtMove[
     \stEnvQTQueueAnnot{\roleP}{\roleQ}{\gtLab[j]}
    ]
    \gtWithTime{\cVali}{
      \gtCommTTransit{\roleP}{\roleQ}{i \in I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtGi[i]}{j}
    }
  }
  \\[2ex]

  \inference[\iruleGtMoveIn]{
    j \in I
    &
   \highlight{\cVal \models \ccstI[j]}
    &
   \highlight{ \cVali = \cValUpd{\cVal}{\crstI[j]}{0}}
  }{
    \gtWithTime{\cVal}{
      \gtCommTTransit{\roleP}{\roleQ}{i \in I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtGi[i]}{j}
    }
    \gtMove[
     \stEnvQTRecvAnnotSmall{\roleQ}{\roleP}{\gtLab[j]}
    ]
    \gtWithTime{\cVali}{\gtGi[j]}
  }\\[2ex]

  \inference[\iruleGtMoveCtx]{
    \forall i \in I :
    \gtWithTime{\cVal}{\gtGi[i]}
    \gtMove[\stEnvAnnotGenericSym]
    \gtWithTime{\cVali}{\gtGii[i]}
    &
    \roleP, \roleQ \notin \ltsSubject{\stEnvAnnotGenericSym}
    &
    \stEnvAnnotGenericSym \neq \timeLab
  }{
    \gtWithTime{\cVal}{
      \gtCommTSmall{\roleP}{\roleQ}{i \in
      I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtGi[i]}
    }
    \gtMove[\stEnvAnnotGenericSym]
    \gtWithTime{\cVali}{
      \gtCommTSmall{\roleP}{\roleQ}{i \in
      I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtGii[i]}
    }
  }\\[2ex]

  \inference[\iruleGtMoveCtxi]{
    \forall i \in I :
    \gtWithTime{\cVal}{\gtGi[i]}
    \gtMove[\stEnvAnnotGenericSym]
    \gtWithTime{\cVali}{\gtGii[i]}
    &
    \roleQ \notin \ltsSubject{\stEnvAnnotGenericSym}
  }{
    \gtWithTime{\cVal}{
      \gtCommTTransit{\roleP}{\roleQ}{i \in
      I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtGi[i]}{j}
     }
    \gtMove[\stEnvAnnotGenericSym]
    \gtWithTime{\cVali}{
      \gtCommTTransit{\roleP}{\roleQ}{i \in
      I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtGii[i]}{j}
    }
  }%

\end{array}
\]
\caption{Timed Global Type Reduction Rules}
\Description{Timed Global Type Reduction Rules}
\label{fig:gtype:red-rules}
\end{figure}


==> typingsystem/label.tex <==
\begin{definition}[Transition Labels]
  \label{def:aatmpst-env-reduction-label}%
  \label{def:aatmpst-label-subject}%
  Let $\stEnvAnnotGenericSym$ %
  be a transition label of the form:
  \[
  \begin{array}{rcll}
  \stEnvAnnotGenericSym &\bnfdef&
   \stEnvQQueueAnnotSmall{\roleP}{\roleQ}{\stLab}&
    \text{(in session $\mpS$, $\roleP$ sends message $\stLab$ to $\roleQ$)}
    \\
    &\bnfsep&
    \stEnvQRecvAnnotSmall{\roleP}{\roleQ}{\stLab}&
    \text{(in session $\mpS$, $\roleP$ receives message $\stLab$ from $\roleQ$)}
    \\
     &\bnfsep&\timeLab&
     \text{(time passing)}
  \end{array}
  \]
\noindent
The subject set of a transition label, written
\,$\ltsSubject{\stEnvAnnotGenericSym}$,\, is defined as follows:
\[
\begin{array}{c}
   \ltsSubject{\stEnvQQueueAnnotSmall{\roleP}{\roleQ}{\stLab}}
    =
    \ltsSubject{\stEnvQRecvAnnotSmall{\roleP}{\roleQ}{\stLab}}
    =
    \setenum{\roleP}
   \quad \qquad
     \ltsSubject{\timeLab} = \emptyset
\end{array}
\]
\end{definition}



==> typingsystem/proj.tex <==
\begin{definition}[Timed Global Type Projection]%
  \label{def:global-proj}%
  \label{def:local-type-merge}%
  The \emph{projection of a timed global type $\gtG$ onto a role $\roleP$}, %
  written $\gtProj{\gtG}{\roleP}$, %
  is:

  \smallskip%
  \centerline{\(%
  \small%
  \begin{array}{c}
    \gtProj{\left(%
      \gtCommTSmall{\roleQ}{\roleR}
      {i \in I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtG[i]}%
      \right)}{\roleP}%
    =\!%
    \left\{%
    \begin{array}{@{}l@{\hskip 2mm}r@{}}
      \stIntSum{\roleR}{i \in I}{ %
        \stTChoice{\stLab[i]}{\stS[i]}{\ccstO[i], \crstO[i]} \stSeq (\gtProj{\gtG[i]}{\roleP})%
      }%
      &\text{\footnotesize%
        if\, $\roleP = \roleQ$%
      }%
      \\[1mm]%
      \stExtSum{\roleQ}{i \in I}{%
        \stTChoice{\stLab[i]}{\stS[i]}{\ccstI[i], \crstI[i]} \stSeq (\gtProj{\gtG[i]}{\roleP})%
      }%
      &\text{\footnotesize%
        if\, $\roleP = \roleR$%
      }%
          \\[2mm]%
      \stMerge{i \in I}{\gtProj{\gtG[i]}{\roleP}}%
      &
      \text{\footnotesize%
        if\, $\roleP \neq \roleQ$\, and \,$\roleP \neq \roleR$%
      }%
    \end{array}
    \right.
    \\[8mm]%
      \gtProj{\left(%
      \gtCommTTransit{\roleQ}{\roleR}
      {i \in I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtG[i]}{j}%
      \right)}{\roleP}%
    =\!%
    \left\{%
    \begin{array}{@{}l@{\hskip 2mm}r@{}}
     \stExtSum{\roleQ}{i \in I}{%
        \stTChoice{\stLab[i]}{\stS[i]}{\ccstI[i], \crstI[i]} \stSeq (\gtProj{\gtG[i]}{\roleP})%
      }%
      &\text{\footnotesize%
        if\, $\roleP = \roleR$%
      }%
   \\[1mm]
      \gtProj{\gtG[j]}{\roleP}
      &\text{\footnotesize%
        if\, $\roleP \neq \roleR$%
      }%
    \end{array}
    \right.
    \\[8mm]%
    \gtProj{(\gtRec{\gtRecVar}{\gtG})}{\roleP}%
    \;=\;%
    \left\{%
    \begin{array}{@{\hskip 0.5mm}l@{\hskip 5mm}l@{}}
      \stRec{\stRecVar}{(\gtProj{\gtG}{\roleP})}%
      &%
      \text{\footnotesize%
        if\,
        $\roleP \in \gtRoles{\gtG}$ \,or\,
        $\fv{\gtRec{\gtRecVar}{\gtG}} \neq \emptyset$%
      }%
      \\%
      \stEnd%
      &%
      \text{\footnotesize%
        otherwise}
    \end{array}
    \right.%
    \quad\qquad%
    \begin{array}{@{}r@{\hskip 1mm}c@{\hskip 1mm}l@{}}
      \gtProj{\gtRecVar}{\roleP}%
      &=&%
      \stRecVar%
      \\%
      \gtProj{\gtEnd}{\roleP}%
      &=&%
      \stEnd%
    \end{array}
  \end{array}
  \)}%
  \smallskip%


  \noindent%
  where
  $\stMerge{}{}$ is %
  the \emph{merge operator for timed session types} %
  (\emph{full merging}):

  \smallskip%
  \centerline{\(%
  \small%
  \begin{array}{l}%
    \textstyle%
    \stExtSum{\roleP}{i \in I}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq \stT[i]}%
    \;\stBinMerge\;%
    \stExtSum{\roleP}{\!j \in J}{\stTChoice{\stLab[j]}{\stSi[j]}{\ccsti[j], \crsti[j]} \stSeq \stTi[j]} = %
    \\
    \stExtSum{\roleP}{k \in I \cap J}{\stTChoice{\stLab[k]}{\stS[k]}{\ccst[k], \crst[k]} \stSeq%
      (\stT[k] \!\stBinMerge\! \stTi[k])%
    }%
    \stExtC%
    \stExtSum{\roleP}{i \in I \setminus J}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq \stT[i]}%
    \stExtC%
    \stExtSum{\roleP}{\!j \in J \setminus I}{\stTChoice{\stLab[j]}{\stSi[j]}{\ccsti[j], \crsti[j]} \stSeq \stTi[j]}%
    \\[3mm]%
    \stIntSum{\roleP}{i \in I}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq \stT[i]}%
    \,\stBinMerge\,%
    \stIntSum{\roleP}{i \in I}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq \stTi[i]}%
    \;=\;%
    \stIntSum{\roleP}{i \in I}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq (\stT[i]
    \stBinMerge \stTi[i])}%
    \\[3mm]%
    \stRec{\stRecVar}{\stT} \,\stBinMerge\, \stRec{\stRecVar}{\stU}%
    \,=\,%
    \stRec{\stRecVar}{(\stT \stBinMerge \stU)}%
    \qquad%
    \stRecVar \,\stBinMerge\, \stRecVar%
    \,=\,%
    \stRecVar%
    \qquad%
    \stEnd \,\stBinMerge\, \stEnd%
    \,=\,%
    \stEnd%
  \end{array}
  \)}%


 The \emph{queue projection}
  of $\gtG$ onto $\roleP$, written $\gtQProj{\gtG}{\roleP}$, is:

   \smallskip%
  \centerline{\(%
  \small
  \begin{array}{c}
   \gtQProj{\left(%
      \gtCommTSmall{\roleQ}{\roleR}
      {i \in I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtG[i]}%
      \right)}{\roleP}%
    =
     \gtQProj{\gtG[i]}{\roleP} \,\,\,
      \text{ \footnotesize if $i \in I$ and $\forall j, k \in I$ with $j \neq k$, $\gtQProj{\gtG[j]}{\roleP} = \gtQProj{\gtG[k]}{\roleP}$}
    \\[2mm]%
      \gtQProj{\left(%
      \gtCommTTransit{\roleQ}{\roleR}
      {i \in I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtG[i]}{j}%
      \right)}{\roleP}%
    =%
    \left\{%
    \begin{array}{@{}l@{\hskip 2mm}l@{}}
      \stQCons{\stQMsg{\roleQ}{\gtLab[j]}{\stS[j]}}{\gtQProj{\gtG[j]}{\roleP}}
      & \text{\footnotesize%
        if\, $\roleP = \roleQ$%
      }%
      \\[1mm]%
       \gtQProj{\gtG[j]}{\roleP}
        &\text{\footnotesize
       otherwise
      }%
    \end{array}
    \right.
  \\[2mm]
     \gtQProj{(\gtRec{\gtRecVar}{\gtG})}{\roleP}
    \;=\;%
    \gtQProj{\gtEnd}{\roleP}
     \;=\;
     \stQEmptyType
  \end{array}
  \)}%
\end{definition}




==> typingsystem/subtyping.tex <==
\begin{definition}[Subtyping]\label{def:subtyping}
The \emph{timed session subtyping relation} $\stSub$ is coinductively defined:
\[
\begin{array}{c}
\cinference[\iruleStSubOut]{
  \forall i \in I
  &
  \stS[i] \stSub \stSi[i]
  &
  \ccst[i] = \ccsti[i]
  &
  \crst[i] = \crsti[i]
  &
  \stT[i] \stSub \stTi[i]
}{
  \stIntSum{\roleP}{i \in I}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq \stT[i]}%
  \stSub
  \stIntSum{\roleP}{i \in I \cup J}{\stTChoice{\stLab[i]}{\stSi[i]}{\ccsti[i], \crsti[i]} \stSeq \stTi[i]}%
}
\\[2mm]
\cinference[\iruleStSubIn]{
  \forall i \in I
  &
  \stSi[i] \stSub \stS[i]
  &
  \ccst[i] = \ccsti[i]
  &
  \crst[i] = \crsti[i]
  &
  \stT[i] \stSub \stTi[i]
}{
  \stExtSum{\roleP}{i \in I \cup J}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq \stT[i]}
  \stSub
  \stExtSum{\roleP}{i \in I}{\stTChoice{\stLab[i]}{\stSi[i]}{\ccsti[i], \crsti[i]} \stSeq \stTi[i]}
}
\\[2mm]%
\cinference[\iruleStSubSort]{\stT \stSub \stTi}{
 \stDelegate{\ccst}{\stT} \stSub \stDelegate{\ccst}{\stTi}
}
\quad
\cinference[\iruleStSubRecL]{
  \stT{}\subst{\stRecVar}{\stRec{\stRecVar}{\stT}} \stSub \stTi
}
{
  \stRec{\stRecVar}{\stT} \stSub \stTi
}
\quad
\cinference[\iruleStSubRecR]{
  \stT \stSub \stTi{}\subst{\stRecVar}{\stRec{\stRecVar}{\stTi}}
}{
  \stT \stSub \stRec{\stRecVar}{\stTi}
}
\\[2mm]
\cinference[\iruleStSubEnd]{}{
  \stEnd \stSub \stEnd
}
\quad
\cinference[\iruleSubEQueueTypeEmpty]{%
    \vphantom{X}%
    }{%
     \stQEmptyType \stSub \stQEmptyType
    }%
\quad
     \cinference[\iruleSubEQueueType]{%
      \stS \stSub \stSi & \stQType \stSub \stQTypei%
    }{%
        \stQCons{\stQMsg{\roleQ}{\gtLab}{\stS}}{\stQType}
         \stSub   \stQCons{\stQMsg{\roleQ}{\gtLab}{\stSi}}{\stQTypei}}%
\end{array}
\]
\end{definition}

==> typingsystem/syntax.tex <==
\begin{figure}[t]%
  \[
    \begin{array}{r@{\quad}c@{\quad}l@{\quad}l}
       \stS& \bnfdef & \stDelegate{\ccst}{\stT}
      & \text{\footnotesize{Session Type}}
      \\
      \gtG & \bnfdef &
      \gtCommT{\roleP}{\roleQ}{i \in
        I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtG[i]}
        &
        {\footnotesize\text{Transmission}} \\
        & \bnfsep &
          \gtCommTTransit{\roleP}{\roleQ}{i \in
          I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtG[i]}{j}~(j \in I)
        &
      \footnotesize\text{Transmission en route (Runtime)} \\
        & \bnfsep & \gtRec{\gtRecVar}{\gtG} \quad \bnfsep \quad \gtRecVar \quad
        \bnfsep \quad \gtEnd &
        \text{\footnotesize Recursion, Type variable, Termination}
       \\[0.5ex]
      \stT
        & \bnfdef & \stExtSum{\roleP}{i \in I}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq \stT[i]}
          & \text{\footnotesize External choice (Receive)} \\
        & \bnfsep & \stIntSum{\roleP}{i \in I}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq \stT[i]}
          & \text{\footnotesize Internal choice (Send)}\\
        & \bnfsep & \stRec{\stRecVar}{\stT} \ \bnfsep \ \stRecVar \
          \bnfsep \ \stEnd &
        \text{\footnotesize Recursion, Type variable, Termination}
        \\
          \stQType
 &\coloncolonequals&%
  \stQCons{\stQMsg{\roleP}{\stLab}{\stS}}{\stQType}%
  \bnfsep \stQEmptyType
  &
   \text{\footnotesize{Queue types}}
    \end{array}
  \]
  \caption{Syntax of types.}
  \Description{Syntax of types.}
  \label{fig:syntax-global-type}%
  \label{fig:syntax-local-type}%
  \label{fig:syntax-aatmpst}
\end{figure}



==> typingsystem/typing_context_reduction.tex <==
\begin{figure}[t]%
  \centerline{\(
  \small
  \begin{array}{c}
     \inference[\iruleTCtxRec]{%
      \stEnv \!\stEnvComp \stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{
      \stCPair{\cVal}{%
        \stT\subst{\stRecVar}{\stRec{\stRecVar}{\stT}}}%
      }%
      \stEnvQTMoveGenAnnotT \stEnvi%
    }{%
      \stEnv \!\stEnvComp \stEnvMap{%
       \mpChanRole{\mpS}{\roleP}
      }{
      \stCPair{\cVal}{%
        \stRec{\stRecVar}{\stT}}%
      }%
      \stEnvQTMoveGenAnnotT \stEnvi%
    }%
    \quad
    \inference[\iruleTCtxCongX]{%
      \stEnv \stEnvQTMoveGenAnnotT \stEnvi
    }{%
      \stEnv \!\stEnvComp \stEnvMap{\mpFmt{x}}{\stCPair{\cVal}{\stT}}
      \stEnvQTMoveGenAnnotT%
      \stEnvi \!\stEnvComp \stEnvMap{\mpFmt{x}}{\stCPair{\cVal}{\stT}}
    }%
    \quad
     \inference[\iruleTCtxCongCombined]{%
      \stEnv \stEnvQTMoveGenAnnotT \stEnvi
      &
   \highlight{ \stTEnvAnnotGenericSymT \neq \timeLab}
    }{%
      \stEnv \!\stEnvComp \stEnvMap{\mpChanRole{\mpS}{\roleP}}{\stSpecf}
      \stEnvQTMoveGenAnnotT%
      \stEnvi \!\stEnvComp \stEnvMap{\mpChanRole{\mpS}{\roleP}}{\stSpecf}}%
\\[2mm]
 \inference[\iruleTCtxSend]
    {k \!\in\! I
     &
    \highlight{\cVal \models \ccst[k]}}
     { \stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{
        \stMPair{
        \stCPair{\cVal}{%
          \stIntSum{\roleQ}{i \in I}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq \stT[i]}}%
        }{%
          \stQType%
        }%
      \;\stEnvQTMoveQueueAnnot{\roleP}{\roleQ}{\stLab[k]}\;%
      \stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{%
        \stMPair{
        \stCPair{\mpFmt{\cValUpd{\cVal}{\crst[k]}{0}}}
          {\stT[k]}%
        }{%
          \stQCons{\stQType}{%
            \stQCons{%
              \stQMsg{\roleQ}{\stLab[k]}{\stS[k]}%
            }{%
              \stQEmptyType%
            }%
          }%
      }}
      }}
      \\[2mm]
      \inference[\iruleTCtxRcv]
       {k \!\in\! I &
      \highlight{\cVal \models \ccst[k]} &
      \stS[k]\!\stSub\!\stSi[k]
}
      {
      \stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{%
       \stQCons{\stQMsg{\roleQ}{\stLab[k]}{\stS[k]}}{\stQType}%
      } %
      \stEnvQComp %
      \stEnvMap{%
        \mpChanRole{\mpS}{\roleQ}%
      }{
      \stCPair{\cVal}{%
          \stExtSum{\roleP}{i \in I}{\stTChoice{\stLab[i]}{\stSi[i]}{\ccst[i], \crst[i]} \stSeq \stT[i]}}%
      }%
      \;\stEnvQTMoveRecvAnnot{\roleQ}{\roleP}{\stLab[k]}\;
      \stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{%
               \stQType
      }%
      \stEnvQComp%
      \stEnvMap{%
        \mpChanRole{\mpS}{\roleQ}%
      }{
        \stCPair{\mpFmt{\cValUpd{\cVal}{\crst[k]}{0}}}%
          {\stT[k]}
          }
          }
 \\[3mm]
   \highlight{\inferenceSingle[\iruleTCtxTimeSession]
      {\stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{\stCPair{\cVal}{%
         \stT}}
       \;\stEnvQTMoveTimeAnnot\;
       \stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{%
          \stCPair{\cVal + \timeLab}{\stT}%
        }}}
      \qquad
          \highlight{ \inferenceSingle[\iruleTCtxTimeCombined]
      { \stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{\stMPair{\stCPair{\cVal}{%
         \stT}}{\stQType}}
       \;\stEnvQTMoveTimeAnnot\;
       \stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{%
          \stMPair{\stCPair{\cVal + \timeLab}{%
         \stT}}{\stQType}%
        }}}
\\[2mm]
\begin{array}{c}
\highlight{ \inferenceSingle[\iruleTCtxTimeQ]
        { \stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{\stQType}
       \;\stEnvQTMoveTimeAnnot\;
       \stEnvMap{%
        \mpChanRole{\mpS}{\roleP}%
      }{%
          \stQType}} }
 \end{array}
 \begin{array}{c}
 \highlight{
 \inference[\iruleTCtxTime]
       {\stEnv[1] \;\stEnvQTMoveTimeAnnot\; \stEnvi[1]
       &  \; { \stEnv[2] \;\stEnvQTMoveTimeAnnot\; \stEnvi[2]}
    }
    {
      \stEnv[1] \stEnvComp \stEnv[2]
          \;\stEnvQTMoveTimeAnnot\;
      \stEnvi[1] \stEnvComp \stEnvi[2]}}
   \quad
    \inference[\iruleTCtxStruct]
       {\stEnv \;\stQEquiv\; \stEnv[1]%
       &
       \stEnv[1] \;\stEnvQTMoveGenAnnotT\; \stEnvi[1]
       &
       \stEnvi[1] \;\stQEquiv\; \stEnvi
       }{\stEnv \;\stEnvQTMoveGenAnnotT\; \stEnvi
     }
     \end{array}
 \end{array}
\)}
  \caption{Typing environment semantics.}
  \label{fig:aat-mpst-semantics-typing-context}%
\end{figure}


==> typingsystem/typing_rules.tex <==
\begin{small}
\begin{figure}[t]
  \hspace{-5mm}%
  \scalebox{0.91}{%
  \begin{minipage}{1.1\linewidth}
\[
  \begin{array}{c}
    \inference[\iruleMPX]{%
      \mpEnvApp{\mpEnv}{X} = \highlight{\stFmt{\stCPair{\cVal[1]}{\stT[1]},\ldots,\stCPair{\cVal[n]}{\stT[n]}}}%
    }{%
      \mpEnvEntails{\mpEnv}{X}{\highlight{\stCPair{\cVal[1]}{\stT[1]},\ldots,\stCPair{\cVal[n]}{\stT[n]}}}%
    }%
    \quad%
    \inference[\iruleMPSub]{
     \highlight{ \stCPair{\cVal}{\stT} \stSub \stCPair{\cVali}{\stTi}}%
    }{%
     \highlight{ \stEnvEntails{\stEnvMap{\mpC}{ \stCPair{\cVal}{\stT}}}{\mpC}{ \stCPair{\cVali}{\stTi}}}%
    }%
       \quad
     \inference[\iruleMPEnd]{
      \forall i \in 1..n%
      &%
     \highlight{ \stEnvEntails{\stEnvMap{\mpC[i]}{\stCPair{\cVal[i]}{\stT[i]}}}{%
        \mpC[i]%
      }{%
        \stCPair{\cVali[i]}{\stEnd}%
      }}%
    }{%
      \highlight{\stEnvEndP{%
        \stEnvMap{\mpC[1]}{\stCPair{\cVal[1]}{\stT[1]}}%
        \stEnvComp \ldots \stEnvComp%
        \stEnvMap{\mpC[n]}{\stCPair{\cVal[n]}{\stT[n]}}%
      }}%
    }%
    \\[3mm]%
    \inference[\iruleMPDef]{%
        \stJudge{%
          \mpEnv \mpEnvComp%
          \mpEnvMap{\mpX}{\highlight{\stCPair{\cVal[1]}{\stT[1]}, \ldots, \stCPair{\cVal[n]}{\stT[n]}}}%
        }{%
          \stEnvMap{x_1}{\highlight{\stCPair{\cVal[1]}{\stT[1]}}}%
          \stEnvComp \ldots \stEnvComp%
          \stEnvMap{x_n}{\highlight{\stCPair{\cVal[n]}{\stT[n]}}}%
        }{%
          \mpP%
        }%
        &%
        \stJudge{%
          \mpEnv \mpEnvComp%
          \mpEnvMap{\mpX}{\highlight{\stCPair{\cVal[1]}{\stT[1]}, \ldots, \stCPair{\cVal[n]}{\stT[n]}}}%
        }{%
          \stEnv%
        }{}{%
          \mpQ%
        }%
    }{%
      \stJudge{\mpEnv}{%
        \stEnv%
      }{%
        \mpDef{\mpX}{%
          \stEnvMap{x_1}{\highlight{\stCPair{\cVal[1]}{\stT[1]}}},%
          \ldots,%
          \stEnvMap{x_n}{\highlight{\stCPair{\cVal[n]}{\stT[n]}}}%
        }{\mpP}{\mpQ}%
      }%
    }%
    \\[3mm]%
      \inference[\iruleMPNil]{%
      \stEnvEndP{\stEnv}%
    }{%
      \stJudge{\mpEnv}{\stEnv}{\mpNil}%
    }%
\qquad
    \inference[\iruleMPCall]{%
        \mpEnvEntails{\mpEnv}{X}{%
         \highlight{ \stCPair{\cVal[1]}{\stT[1]},\ldots, \stCPair{\cVal[n]}{\stT[n]}}%
        }%
        &%
        \stEnvEndP{\stEnv[0]}%
        &%
        \forall i \in 1..n%
        &%
        \stEnvEntails{\stEnv[i]}{\mpC[i]}{\highlight{\stCPair{\cVal[i]}{\stT[i]}}}%
    }{%
      \stJudge{\mpEnv}{%
        \stEnv[0] \stEnvComp%
        \stEnv[1] \stEnvComp \ldots \stEnvComp \stEnv[n]%
      }{%
        \mpCall{\mpX}{\mpC[1],\ldots,\mpC[n]}%
      }%
    }%
    \\[3mm]%
        \inference[\iruleMPClock]{%
     \highlight{\forall \cUnit \in \ccst:}
     &
         \highlight{\stJudge{\mpEnv}{%
        \stEnvQ }{\delay{\cUnit}{\mpP}}}}%
    {%
      \highlight{\stJudge{\mpEnv}{%
        \stEnvQ }{\delay{\ccst}{\mpP}} }
      }%
    \qquad
      \inference[\iruleMPTime]{%
     \highlight{ \stJudge{\mpEnv}{%
        \stEnvQ \,\tcFmt{+}\, \cUnit%
      }{%
        \mpP%
      }}%
      }{\highlight{%
     \stJudge{\mpEnv}{%
        \stEnvQ }{\delay{\cUnit}{\mpP}} }
    }%
    \\[3mm]%
    \inference[\iruleMPBranch]{
    \begin{array}{c}
   \highlight{ \forall i \!\in\! I \,\,\,
    \forall \cUnit:
    \cUnit \leq n \Longrightarrow \cVal + \cUnit \models \ccst[i] }
    \\[0.5mm]
      \highlight{ \forall i \!\in\! I:
        \stEnvEntails{\stEnv[1]}{\mpC}{%
         \stCPair{\cVal}{ \stExtSum{\roleQ}{i \in I}{\stTChoice{\stLab[i]}{\stS[i]}{\ccst[i], \crst[i]} \stSeq \stT[i]}}%
        }}%
        \quad
       \highlight{ \stS[i] = \stCPair{\ccsti[i]}{\stTi[i]}}
      \quad
       \highlight{ \cVali[i] \models \ccsti[i]}
        \\[0.5mm]
       \highlight{ \forall i \!\in\! I \,\,
       \forall \cUnit \leq n:
       \stJudge{\mpEnv}{%
          \stEnvQ \,\tcFmt{+}\, \cUnit \stEnvComp%
          \stEnvMap{y_i}{\stCPair{\cVali[i]}{\stTi[i]}} \stEnvComp%
          \stEnvMap{\mpC}{\stCPair{\cValUpd{\cVal + \cUnit}{\crst[i]}{0}}{\stT[i]}}%
        }{%
          \mpP[i]%
        }}
        \end{array}
    }{%
      \highlight{\stJudge{\mpEnv}{%
        \stEnv \stEnvComp \stEnv[1]%
      }{%
        \mpTBranch{\mpC}{\roleQ}{i \in I}{\mpLab[i]}{y_i}{\mpP[i]}{n}{}%
      }}%
    }%
    \\[3mm]%
    \inference[\iruleMPSel]{%
      \begin{array}{c}
    \highlight{\forall \cUnit:   \cUnit \leq n \Longrightarrow \cVal + \cUnit \models \ccst }
      \\[0.5mm]
    \highlight{\stEnvEntails{\stEnv[1]}{\mpC}{%
       \stCPair{\cVal}{ \stIntSum{\roleQ}{}{\stTChoice{\stLab}{\stS}{\ccst, \crst} \stSeq \stT}}}}%
      \quad
    \highlight{\stS = \stDelegate{\ccsti}{\stTi}}
      \quad
\highlight{\stEnvEntails{\stEnv[2]}{\mpD}{\stCPair{\cVali}{\stTi}}}%
     \quad
     \highlight{\cVali \models \ccsti}
    \\[0.5mm]
    \highlight{\forall \cUnit \leq n:  \stJudge{\mpEnv}{%
        \stEnvQ \,\tcFmt{+}\, \cUnit \stEnvComp \stEnvMap{\mpC}{\stCPair{\cValUpd{\cVal + \cUnit}{\crst}{0}}{\stT}}%
      }{%
        \mpP%
      }
      }%
      \end{array}
    }{%
      \highlight{\stJudge{\mpEnv}{%
        \stEnv \stEnvComp \stEnv[1] \stEnvComp \stEnv[2]%
      }{%
        \mpTSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}{n}%
      }}%
    }%
    \\[3mm]%
      \inference[\iruleMPPar]{%
      \stJudge{\mpEnv}{%
        \stEnvQ[1]%
      }{%
        \mpP[1]%
      }%
      &%
      \stJudge{\mpEnv}{%
        \stEnvQ[2]%
      }{%
        \mpP[2]%
      }%
    }{%
      \stJudge{\mpEnv}{%
        \stEnvQ[1] \stEnvQComp \stEnvQ[2]%
      }{%
        \mpP[1] \mpPar \mpP[2]%
      }%
    }%
    \quad
    \inference[\iruleMPKill]{%
     \stEnvEndP{\stEnv}
      &%
     n \geq 0
      }%
    {%
      \stJudge{\mpEnv}{%
        \stEnvQ \stEnvQComp \highlight{\stEnvMap{%
          \mpChanRole{\mpS}{\roleP[1]}%
        }{%
           \stSpecf[1]
        }
        \stEnvQComp
        \ldots
         \stEnvQComp \stEnvMap{%
          \mpChanRole{\mpS}{\roleP[n]}%
        }{%
        \stSpecf[n]
        }}%
      }{%
       \kills{\mpS}%
      }%
    }%
    \\[3mm]
      \inference[\iruleMPTry]{%
      \stJudge{\mpEnv}{%
        \stEnvQ%
      }{%
        \mpP%
      }%
      &%
      \procSubject{\mpP} = \setenum{\mpC}
      &
      \stJudge{\mpEnv}{%
        \stEnvQ%
      }{%
        \mpQ%
      }%
    }{%
      \stJudge{\mpEnv}{%
        \stEnvQ%
      }{%
         \trycatch{\mpP}{\mpQ}
      }%
    }%
          \\[3mm]
    \inference[\iruleMPCancel]{%
      \stJudge{\mpEnv}{%
        \stEnvQ%
      }{%
        \mpQ%
      }%
      }{%
      \stJudge{\mpEnv}{%
        \stEnvQ%
         \stEnvQComp
          \highlight{\stEnvMap{%
         \mpChanRole{\mpS}{\roleP}
        }{%
           \stSpecf
        }}
      }{%
         \mpCancel{\mpChanRole{\mpS}{\roleP}}{\mpQ}
      }%
    }%
    \qquad
 \inference[\iruleMPFailed]
 {\highlight{
 \procSubject{\mpP} %
 \subseteq \dom{\stEnvQ}}}
    {\highlight{\stJudge{\mpEnv}{%
        \stEnvQ }{\mpFailedP{\mpP}}}}
\\[3mm]
  \inference[\iruleMPResProp]{%
      \stEnvQi = \setenum{%
        \stEnvMap{\mpChanRole{\mpS}{\roleP}}{\highlight{\stSpecf[\roleP]}}}_{\roleP \in I} %
      &%
      \mpS \not\in \stEnvQ%
      &%
  \highlight{\predPApp{\stUntimed{\stEnvQi}}}
      &%
      \stJudge{\mpEnv}{%
        \stEnvQ \stEnvQComp \stEnvQi%
      }{%
        \mpP%
      }%
    }{%
      \stJudge{\mpEnv}{%
        \stEnvQ%
      }{%
        \mpRes{\stEnvMap{\mpS}{\stEnvi}}\mpP%
      }%
    }%
    \\[3mm]
     \inference[\iruleMPResPropG]{%
    \highlight{ \stEnvAssoc{\gtWithTime{\cVal}{\gtG}}{\stEnv[\gtG]}}
       &%
      \dom{\stEnv[\gtG]} = \mpS \not\in \stEnvQ%
      &%
      \stJudge{\mpEnv}{%
        \stEnvQ \stEnvQComp \stEnvQ[\gtG]%
      }{%
        \mpP%
      }%
    }{%
      \stJudge{\mpEnv}{%
        \stEnvQ%
      }{%
        \mpRes{\stEnvMap{\mpS}{\stEnv[\gtG]}}\mpP%
      }%
    }%
 \\[3mm]%
    \hdashline%
    \\[-1mm]%
        \inference[\iruleMPQueueEmpty]{\stEnvEndP{\stEnvQ}}{%
     \highlight{ \stJudge{\mpEnv}{\stEnvQ \stEnvQComp %
        \stEnvMap{%
          \mpChanRole{\mpS}{\roleP}%
        }{%
          \stQEmptyType%
        }%
      }{%
        \mpSessionQueueO{\mpS}{\roleP}{\mpQueueEmpty}%
      }}%
    }%
    \qquad%
    \inference[\iruleMPQueue]{%
     \highlight{ \stJudge{\mpEnv}{\stEnvQ}{%
        \mpSessionQueueO{\mpS}{\roleP}{%
          \mpQueue%
        }%
      }}%
      &%
    \highlight{  \stS = \stCPair{\ccst}{\stT}}
      &
     \highlight{ \cVal \models \ccst}
      &
     \highlight{ \stEnvEntails{\stEnvi}{\mpChanRole{\mpSi}{\roleR}}{\stCPair{\cVal}{\stT}}}%
    }{%
     \highlight{ \stJudge{\mpEnv}{%
        \stEnvUpd{\stEnvQ}{\mpChanRole{\mpS}{\roleP}}{%
          \stQCons{\stQMsg{\roleQ}{\stLab}{\stS}}{\stEnvApp{\stEnvQ}{\mpChanRole{\mpS}{\roleP}}}%
        }
        \stEnvQComp%
        \stEnvi%
      }{%
        \mpSessionQueueO{\mpS}{\roleP}{%
          \mpQueueCons{%
            \mpQueueOElem{\roleQ}{\mpLab}{\mpChanRole{\mpSi}{\roleR}}%
          }{%
            \mpQueue%
          }%
        }
      }%
    }}%
\end{array}
\]
  \end{minipage}
}
  \caption[\ATMP typing rules]{%
   \ATMP typing rules: processes (top) and queues (bottom). %
  }%
  \label{fig:aat-mpst-rules}%
  \label{def:aat-mpst-env-comp-queue}%
\end{figure}
\end{small}



==> updated_theory/queue_projection.tex <==
 \begin{definition}[Queue Projection]
 \label{def:queue_proj}
 The \emph{queue projection 
  of a timed global type $\gtG$ onto a role $\roleP$}, written as $\gtQProj{\gtG}{\roleP}$, is:

   \smallskip%
  \centerline{\(%
  \small
  \begin{array}{c}
   \gtQProj{\left(%
      \gtCommTSmall{\roleQ}{\roleR}
      {i \in I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtG[i]}%
      \right)}{\roleP}%
    =
     \gtQProj{\gtG[i]}{\roleP} \,\,\,
      \text{ \footnotesize $i \in I$}
    \\[2mm]%
      \gtQProj{\left(%
      \gtCommTTransit{\roleQ}{\roleR}
      {i \in I}{\gtLab[i]}{\stS[i]}{\ccstO[i], \crstO[i], \ccstI[i], \crstI[i]}{\gtG[i]}{j}%
      \right)}{\roleP}%
    =%
    \left\{%
    \begin{array}{@{}l@{\hskip 2mm}l@{}}
      \stQCons{\stQMsg{\roleQ}{\gtLab[j]}{\stS[j]}}{\gtQProj{\gtG[j]}{\roleP}}
      & \text{\footnotesize%
        if\, $\roleP = \roleQ$%
      }%
      \\[1mm]%
       \gtQProj{\gtG[j]}{\roleP}
        &\text{\footnotesize
       otherwise
      }%
    \end{array}
    \right.
  \\[2mm]
     \gtQProj{(\gtRec{\gtRecVar}{\gtG})}{\roleP}
    \;=\;%
    \gtQProj{\gtEnd}{\roleP}
     \;=\;
     \stQEmptyType
  \end{array}
  \)}%
  \end{definition}

